A Two-Time-Scale Stochastic Optimization Framework with Applications in Control and Reinforcement Learning

We study a new two-time-scale stochastic gradient method for solving optimization problems, where the gradients are computed with the aid of an auxiliary variable under samples generated by time-varying MDPs controlled by the underlying optimization variable. These time-varying samples make gradient directions in our update biased and dependent, which can potentially lead to the divergence of the iterates. In our two-time-scale approach, one scale is to estimate the true gradient from these samples, which is then used to update the estimate of the optimal solution. While these two iterates are implemented simultaneously, the former is updated "faster" than the latter. Our first contribution is to characterize the finite-time complexity of the proposed two-time-scale stochastic gradient method. In particular, we provide explicit formulas for the convergence rates of this method under different structural assumptions, namely, strong convexity, PL condition, and general non-convexity. We apply our framework to various policy optimization problems. First, we look at the infinite-horizon average-reward MDP with finite state and action spaces and derive a convergence rate of $O(k^{-2/5})$ for the online actor-critic algorithm under function approximation, which recovers the best known rate derived specifically for this problem. Second, we study the linear-quadratic regulator and show that an online actor-critic method converges with rate $O(k^{-2/3})$. Third, we use the actor-critic algorithm to solve the policy optimization problem in an entropy regularized Markov decision process, where we also establish a convergence of $O(k^{-2/3})$. The results we derive for both the second and third problem are novel and previously unknown in the literature. Finally, we briefly present the application of our framework to gradient-based policy evaluation algorithms in reinforcement learning.

==> Supplementary_Proof_Corollary.tex <==


\section{Proof Sketch of Corollary \ref{cor:LQR}}\label{sec:cor:LQR}

In this section, we briefly sketch how the analysis of Theorem \ref{thm:convergence_decision_pl} can be extended to proving Corollary \ref{cor:LQR}. We note that Assumption \ref{assump:stable_K} can be shown to imply Assumptions \ref{assump:HG_smooth}-\ref{assump:tv_bound} of the general optimization framework as discussed in Section \ref{sec:applications_lqr}.
% 
The main difference between Theorem \ref{thm:convergence_decision_pl} and Corollary \ref{cor:LQR} is that Theorem \ref{thm:convergence_decision_pl} assumes the access to a stochastic oracle that tracks the gradient of the objective function \eqref{operator:H}, whereas in the LQR problem, we use a stochastic oracle $H$ that tracks the natural gradient\vspace{-3pt}
\begin{align*}
    \Eset_{X\sim\mu_{\theta}}[H(\theta,\omega^{\star}(\theta),X)]=\Ical_{\theta}^{-1}\nabla f(\theta),
\end{align*}
where $\Ical_{\theta}$ denotes the Fisher information matrix under $\theta$.\vspace{-5pt}
% Defining
% \begin{align*}
% \widebar{\Delta H_k} &\triangleq H(\theta_k,\omega_k,X_k)-H(\theta_k,\omega^{\star}(\theta_k),X_k),\\
% % \Gamma_H(\theta, X) &\triangleq\left\langle\nabla f(\theta),H(\theta,\omega^{\star}(\theta),X)-\mathbb{E}_{\hat{X}\sim\mu_{\theta}}[H(\theta,\omega^{\star}(\theta),\hat{X})]\right\rangle,
% \Delta H_k &\triangleq H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})],
% \end{align*}
By the smoothness of $f$,
% \begin{align}
%     f(\theta_{k+1})&\leq f(\theta_{k})+\langle\nabla f(\theta_k),\theta_{k+1}-\theta_k\rangle+\frac{L_f}{2}\|\theta_{k+1}-\theta_k\|^2\notag\\
%     &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),F(\theta_k,\omega_k,X_k)\rangle+\frac{L_f \alpha_k^2}{2}\|F(\theta_k,\omega_k,X_k)\|^2\notag\\
%     &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),F(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle\notag\\
%     &\hspace{20pt}-\alpha_k\langle\nabla f(\theta_k),\Delta F(\theta_k, \omega_k, X_k)\rangle+\frac{L_f \alpha_k^2}{2}\|F(\theta_k,\omega_k, X_k)\|^2\notag\\
%     &= f(\theta_{k})-\alpha_k\Gamma(\theta_k,X_k)-\alpha_k\langle\nabla f(\theta_k),\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[F(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\notag\\
%     &\hspace{20pt}-\alpha_k\left\langle\nabla f(\theta_k), \Delta F(\theta_k,\omega_k, X_k)\right\rangle+\frac{L_f \alpha_k^2}{2}\|F(\theta_k,\omega_k, X_k)\|^2\notag\\
%     &= f(\theta_{k})-\alpha_k\Gamma(\theta_k,X_k)-\alpha_k\left\langle \nabla f(\theta_k),\Ical_k^{-1}\nabla f(\theta_k)\right\rangle\notag\\
%     &\hspace{20pt}-\alpha_k\left\langle\nabla f(\theta_k), \Delta F(\theta_k,\omega_k, X_k)\right\rangle+\frac{L_f \alpha_k^2}{2}\|F(\theta_k,\omega_k, X_k)\|^2\notag\\
%     &\leq f(\theta_{k})-\alpha_k\Gamma(\theta_k,X_k)-\frac{\alpha_k}{\sigma_u}\left\|\nabla f(\theta_k)\right\|^2-\alpha_k\left\langle\nabla f(\theta_k), \Delta F(\theta_k,\omega_k, X_k)\right\rangle\notag\\
%     &\hspace{20pt}+\frac{L_f \alpha_k^2}{2}\|F(\theta_k,\omega_k, X_k)\|^2,
%     \label{cor:LQR:eq1}
% \end{align}
\begin{align}
    f(\theta_{k+1})&\leq f(\theta_{k})+\langle\nabla f(\theta_k),\theta_{k+1}-\theta_k\rangle+\frac{L}{2}\|\theta_{k+1}-\theta_k\|^2\notag\\
    &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega_k,X_k)\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k,X_k)\|^2\notag\\
    % &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle\notag\\
    % &\hspace{20pt}-\alpha_k\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    % &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),\Delta H_k\rangle-\alpha_k\langle\nabla f(\theta_k),\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\notag\\
    % &\hspace{20pt}-\alpha_k\left\langle\nabla f(\theta_k), \widebar{\Delta H_k}\right\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\notag\\
    &\hspace{20pt}-\alpha_k\left\langle \nabla f(\theta_k),\Ical_k^{-1}\nabla f(\theta_k)\right\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    &\leq f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\notag\\
    &\hspace{20pt}-\frac{\alpha_k}{\sigma_u}\left\|\nabla f(\theta_k)\right\|^2+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2,
    \label{cor:LQR:eq1}
\end{align}
where the last inequality follows from the fact that the Fisher information matrix has upper bounded eigenvalue as implied by Lemma \ref{lem:bounded_sigma_SigmaK}. Comparing \eqref{cor:LQR:eq1} with \eqref{prop:pl_nonconvex:eq1} which is established under the general framework, we note that most terms of \eqref{cor:LQR:eq1} can be handled in similar manners as in Proposition \ref{prop:pl_nonconvex}. 
% we note that the terms $\left\langle\nabla f(\theta_k), \Delta H\right\rangle$, $\left\langle\nabla f(\theta_k), \widebar{\Delta H}\right\rangle$, and $\|H(\theta_k,\omega_k, X_k)\|^2$ can all be handled in similar manners as in Proposition \ref{prop:pl_nonconvex}.
The third term in \eqref{cor:LQR:eq1} has an extra scaling factor $\sigma_u^{-1}$ that does not appear in \eqref{prop:pl_nonconvex:eq1}, which essentially has to be absorbed into $\alpha_k$ and results in a scaled choice of the step size. The rest of the proof proceeds in the same way as the proof of Proposition \ref{prop:pl_nonconvex} and Theorem \ref{thm:convergence_decision_pl}.


==> Supplementary_Proof_Lemma.tex <==
\section{Proof of Lemmas}




% \qed


% \subsection{Proof of Lemma \ref{lem:bound_sum_integral}}
% We upper bound the summation by the integral
% \begin{gather*}
%     \sum_{t=0}^{k}\frac{1}{(t+1)^{u}}\leq \int_{0}^{k+1}\left(\frac{1}{t}\right)^{u} dt=\frac{(k+1)^{1-u}}{1-u},\quad\forall u\in(0,1),\\
%     \sum_{t=0}^{k}\frac{1}{(t+1)^{u}}\leq 1+\int_{1}^{k+1}\frac{1}{t} dt\leq 1+\log(k+1)\leq \frac{\log(k+2)}{\log(2)}.
% \end{gather*}
% Similarly, we have the lower bound
% \begin{align*}
%     \sum_{t=0}^{k}\frac{1}{(t+1)^{u}}\geq \int_{0}^{k}\left(\frac{1}{t+1}\right)^{u} dt\geq\frac{(k+2)^{1-u}-1}{1-u}
%     % \geq (1-\frac{1}{2^{1-u}})\frac{(k+2)^{1-u}}{1-u}
%     \geq (1-\frac{1}{2^{1-u}})\frac{(k+1)^{1-u}}{1-u}.
% \end{align*}

% For $u>1$, we have
% \begin{align*}
%     \sum_{t=0}^{k}\frac{1}{(t+1)^{u}}\leq 1+\int_{1}^{k+1}\left(\frac{1}{t}\right)^{u} dt\leq 1+\frac{1}{u-1}=\frac{u}{u-1}.
% \end{align*}

% In addition,
% \begin{align*}
%     \sum_{t=0}^{k}\frac{\log^2(t+1)}{(t+1)^{u}}&\leq 1+\int_{1}^{k+1}\left(\frac{\log^2(t)}{t}\right)^{u} dt\notag\\
%     &= 1+\frac{2-(k+1)^{1-u}((u-1) \log (k+1)((u-1) \log (k+1)+2)+2)}{(u-1)^{3}}\notag\\
%     &\leq 1+\frac{2}{(u-1)^{3}}=\frac{(u-1)^{3}+2}{(u-1)^{3}}.
% \end{align*}



% For $u\in[-1,0)$, we have
% \begin{align*}
%     \sum_{t=0}^{k}\frac{1}{(t+1)^{u}}&\leq 1+\int_{1}^{k+1}t^{-u} dt= 1+\frac{(k+1)^{1-u}-1}{1-u}\\
%     &=\frac{(k+1)^{1-u}-u}{1-u}\leq \frac{2(k+1)^{1-u}}{1-u},
% \end{align*}
% where the last inequality follows from $-u\leq 1\leq (k+1)^{1-u}$.

% In addition,
% \begin{align*}
%     \sum_{t=0}^{k}\frac{1}{(t+1)^{u}}\leq 1+\int_{1}^{k+1}\frac{1}{t} dt\leq 1+\log(k+1)\leq \frac{\log(k+2)}{\log(2)}.
% \end{align*}

% \qed

% \subsection{Proof of Lemma \ref{lem:G_affinelybounded_D}}
% By Assumption \ref{assump:HG_smooth} we have for all $\theta\in\mathbb{R}^d$ and $\omega\in\mathbb{R}^r$
% \begin{align*}
%     \|G(\theta,\omega,X)\|-\|G(0,0,X)\|\leq \|G(\theta,\omega,X)-G(0,0,X)\|\leq L\left(\|\theta\|+\|\omega\|\right).
% \end{align*}
% Re-arranging terms, we have
% \begin{align*}
%     \|G(\theta,\omega,X)\|\leq \|G(0,0,X)\|+L\left(\|\theta\|+\|\omega\|\right)&\leq D+D\left(\|\theta\|+\|\omega\|\right)\leq D(\|\theta\|+\|\omega\|+1).
% \end{align*}


% By Assumption \ref{assump:Lipschitz_omega}, we have for all $\theta\in\mathbb{R}^d$
% \begin{align*}
%     \|\omega^{\star}(\theta)\|-\|\omega^{\star}(0)\|\leq \|\omega^{\star}(\theta)-\omega^{\star}(0)\|\leq L\|\theta\|.
% \end{align*}
% Re-arranging the terms leads to
% \begin{align*}
%     \|\omega^{\star}(\theta)\|\leq L\|\theta\|+\|\omega^{\star}(0)\|\leq D\|\theta\|+D=D(\|\theta\|+1).
% \end{align*}


% % \qed




\subsection{Proof of Lemma \ref{lem:Lambda_bound}}
Since our Markov processes are time-varying (they depend on the iterates $\theta$), one cannot directly utilize Assumption \ref{assump:markov-chain} to analyze the bias of $G$ in Algorithm \ref{Alg:two-time-scale-SGD} since the mixing time is defined for a fixed Markov chain (see Definition \ref{def:mixing_time}). To handle this difficulty, we introduce the following auxiliary Markov chain $\{\widetilde{X}_{k}\}$ generated under the decision variable $\theta_{k-\tau_k}$ starting from $X_{k-\tau_{k}}$ as follows
\begin{align}
% X_{k-\tau_k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  
{X}_{k-\tau_k} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \widetilde{X}_{k-\tau_k+1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \cdots \widetilde{X}_{k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \widetilde{X}_{k}.
\label{eq:def_distribution_d}
\end{align}
% and we use $d_k$ to denote the distribution of $\widetilde{X}_{k}$. 
% Thus, one can apply Assumption \ref{assump:markov-chain} to $\{\widetilde{X}_{k}\}$. 
For clarity, recall the time-varying Markov processes $\{X_k\}$ generated by Algorithm~\ref{Alg:two-time-scale-SGD}
\begin{align*}
% X_{k-\tau_k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow} 
X_{k-\tau_k} \stackrel{\theta_{k-\tau_k+1}}{\longrightarrow} X_{k-\tau_k+1} \stackrel{\theta_{k-\tau_k+2}}{\longrightarrow} \cdots \stackrel{\theta_{k-1}}{\longrightarrow} X_{k-1} \stackrel{\theta_{k}}{\longrightarrow} X_{k}.
\end{align*}
Recall $z_{k} = \omega_{k} - \omega^{\star}(\theta_{k})$. We define the following quantities
% defined over $X_{k}$ and $\widetilde{X}_{k}$
\begin{align*}
    &T_{1}=\mathbb{E}[\langle\omega_{k}-\omega_{k-\tau_k}, G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\rangle],\notag\\
    &T_{2}=\mathbb{E}[\langle\omega^{\star}(\theta_{k-\tau_k})-\omega^{\star}(\theta_k), G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\rangle],\notag\\
    &T_{3}=\mathbb{E}[\langle z_{k-\tau_k},G(\theta_k,\omega_k,X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)\rangle],\notag\\
    &T_{4}=\mathbb{E}[\langle z_{k-\tau_k}, G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)\rangle],\notag\\
    &T_{5}=\mathbb{E}[\langle z_{k-\tau_k}, G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)-\mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]\rangle],\notag\\
    &T_{6}=\mathbb{E}[\langle z_{k-\tau_k}, \mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\hat{X})]\rangle],\notag\\
    &T_{7}=\mathbb{E}[\langle z_{k-\tau_k}, \mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\hat{X})]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_{k},\omega_{k},\hat{X})]\rangle].
\end{align*}
It is easy to see that
\begin{align}
    \mathbb{E}[\langle\omega_k-\omega^{\star}(\theta_k), \Delta G_k\rangle] 
    % &= \mathbb{E}\big[\langle\omega_k-\omega^{\star}(\theta_k), G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\rangle\big]\notag\\
    % &=\mathbb{E}\big[\big\langle\omega_k-\omega^{\star}(\theta_k), G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\big\rangle\big]\notag\\
    % &=\mathbb{E}\big[\big\langle\omega_k-\omega_{k-\tau_k}, G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\big\rangle\big]\notag\\
    % &\hspace{20pt}+\mathbb{E}\big[\big\langle\omega^{\star}(\theta_{k-\tau_k})-\omega^{\star}(\theta_k), G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\big\rangle\big]\notag\\
    % &\hspace{20pt}+\mathbb{E}\big[\big\langle\omega_{k-\tau_k}-\omega^{\star}(\theta_{k-\tau_k}), G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\big\rangle\big]\notag\\
    &=T_{1}+T_{2}+T_{3}+T_{4}+T_{5}+T_{6}+T_{7}.\label{lem:Lambda_bound:Eq0}
\end{align}
We analyze the terms of \eqref{lem:Lambda_bound:Eq0} individually. First, using \eqref{eq:G_affinelybounded_D} we consider
\begin{align*}
    T_{1}&\leq \mathbb{E}[\|\omega_k-\omega_{k-\tau_k}\|\|G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\|]\notag\\
    &\leq \mathbb{E}\big[\|\omega_k-\omega_{k-\tau_k}\|\left(\|G(\theta_k,\omega_k,X_k)\|+\|\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\|\right)\big]\notag\\
    &\leq 2D\mathbb{E}\big[\|\omega_k-\omega_{k-\tau_k}\|\left(\|\theta_k\|+\|\omega_k\|+1\right)\big],
\end{align*}
which combined with Lemma \ref{lem:omega_k-omega_k-tau} gives
\begin{align}
    T_{1} &\leq 6D^2\beta_{k-\tau_k}\tau_k\mathbb{E}\big[\left(\|\theta_k\|+\|\omega_k\|+1\right)^2\big]\leq 18D^2\beta_{k-\tau_k}\tau_k\mathbb{E}\big[\|\theta_k\|^2+\|\omega_k\|^2+1\big].\label{lem:Lambda_bound:eq1a}    
\end{align}
Similarly, using Assumption \ref{assump:Lipschitz_omega} we bound $T_2$ as
\begin{align}
    &T_{2}\leq \mathbb{E}[\|\omega^{\star}(\theta_{k-\tau_k})-\omega^{\star}(\theta_k)\|\| G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]\|]\notag\\
    % &\leq 2D\mathbb{E}\big[\|\omega^{\star}(\theta_{k-\tau_k})-\omega^{\star}(\theta_k)\|\left(\|\theta_k\|+\|\omega_k\|+1\right)\big]\notag\\
    &\leq 2DL\mathbb{E}[\|\theta_k\hspace{-2pt}-\hspace{-2pt}\theta_{k-\tau_k}\|\left(\|\theta_k\|\hspace{-2pt}+\hspace{-2pt}\|\omega_k\|\hspace{-2pt}+\hspace{-2pt}1\right)]\hspace{-2pt}=\hspace{-2pt} 2DL\mathbb{E}\big[\big\|\hspace{-4pt}\sum_{t=k-\tau_{k}}^{k-1}\hspace{-5pt}\alpha_{t}H(\theta_{t},\omega_{t},H_{t})\big\|\hspace{-1pt}(\|\theta_k\|\hspace{-2pt}+\hspace{-2pt}\|\omega_k\|\hspace{-2pt}+\hspace{-2pt}1)\hspace{-1pt}\big]\notag\\
    &\leq 2DB L\tau_k\alpha_{k-\tau_k}\mathbb{E}[\|\theta_k\|+\|\omega_k\|+1]\leq DB L\tau_k\alpha_{k-\tau_k} \mathbb{E}[\|\theta_k\|^2+\|\omega_k\|^2+4],\label{lem:Lambda_bound:eq1b}    
\end{align}
where the equality is due to \eqref{alg:update_theta}, the third inequality follows from \eqref{assump:H_bounded}, and the last inequality applies $2c\leq c^2+1$ for any scalar $c$. Using Assumption \ref{assump:HG_smooth}, \eqref{assump:H_bounded}, and Lemma \ref{lem:omega_k-omega_k-tau} we analyze $T_3$ in a similar way
\begin{align}
T_{3} &\leq\mathbb{E}\big[\|z_{k-\tau_k}\|\|G(\theta_k,\omega_k,X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)\|\big]\notag\\
&\leq L\mathbb{E}\big[\|z_{k-\tau_k}\|\left(\|\theta_k-\theta_{k-\tau_k}\|+\|\omega_k-\omega_{k-\tau_k}\|\right)\big]\notag\\
&\leq L B\tau_k\alpha_{k-\tau_k}\mathbb{E}\big[\|z_{k-\tau_k}\|\big]+3L D\beta_{k-\tau_k}\tau_k\mathbb{E}\big[\|z_{k-\tau_k}\|\left(\|\omega_k\|+\|\theta_{k}\|+1\right)\big]\notag\\
&\leq \frac{L B\tau_k\alpha_{k-\tau_k}}{2}\mathbb{E}\big[\|z_{k-\tau_k}\|^2+1\big]+\frac{3L D\beta_{k-\tau_k}\tau_k}{2}\mathbb{E}\big[\|z_{k-\tau_k}\|^2+\left(\|\omega_k\|+\|\theta_{k}\|+1\right)^2\big]\notag\\
&\leq 2L D\tau_k\beta_{k-\tau_k}\mathbb{E}\big[\|z_{k-\tau_k}\|^2\big]\hspace{-2pt}+\hspace{-2pt}\frac{9L D\tau_k\beta_{k-\tau_k}}{2}\mathbb{E}\big[\|\omega_k\|^2\hspace{-2pt}+\hspace{-2pt}\|\theta_{k}\|^2\big]\hspace{-2pt}+\hspace{-2pt}5L D\tau_k\beta_{k-\tau_k},\label{lem:Lambda_bound:eq1c}    
\end{align}
where the last inequality follows from $\alpha_k\leq\beta_k$ for all $k\geq 0$. To analyze $T_{4}$, we utilize the law of total expectation: given $\Fcal\subseteq\Fcal'$ and a random variable $X$ we have $\Eset[X\mid\Fcal] = \Eset[\Eset[X\mid\Fcal']\mid\Fcal]$.   

Let $\Fcal_k$ be $\Fcal_k=\{X_0,\ldots,X_k,\theta_0,\ldots,\theta_k,\omega_0,...,\omega_k\}$,
and for convenience we denote
\[p_{k}(x) = P(X_{k} = x\mid\Fcal_{k-1})\quad  \text{and}\quad  \tilde{p}_{k}(x) = P(\widetilde{X}_{k} = x\mid\Fcal_{k-1}).\]
Then, by the Cauchy-Schwarz inequality we have
\begin{align*}
    &\mathbb{E}[\langle z_{k-\tau_k}, G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)\rangle\mid\Fcal_{k-\tau_k}]\notag\\
    % &=\left\langle z_{k-\tau_k}, \mathbb{E}\big[G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)\mid\Fcal_{k-\tau_k}\big]\right\rangle\notag\\
    &\leq\left\|z_{k-\tau_k}\right\| \left\|\mathbb{E}\big[ G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)\mid\Fcal_{k-\tau_k}\big]\right\|\notag\\
    % &=\left\|z_{k-\tau_k}\right\| \left\|\mathbb{E}\left[\Eset\left[ G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)\mid \Fcal_{k-1}\right] \mid\Fcal_{k-\tau_k}\right]\right\|\notag\\
    &=\left\|z_{k-\tau_k}\right\| \Big\|\Eset\Big[\int_{\Xcal}G(\theta_{k-\tau_k},\omega_{k-\tau_k},x)(p_{k}(x)-\tilde{p}_{k}(x))dx \mid\Fcal_{k-\tau_{k}}\Big]\Big\|\notag\\
    &\leq 2D\left\|z_{k-\tau_k}\right\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)\big\|\Eset\big[d_{TV}(p_{k}(\cdot),\tilde{p}_{k}(\cdot))\mid \Fcal_{k-\tau_k}\big],
\end{align*}
where the last inequality uses the definition of the TV distance in \eqref{eq:TV_def}. Recursively applying Assumption \ref{assump:tv_bound}, we obtain from the preceding relation
\begin{align}
&\mathbb{E}\big[\left\langle z_{k-\tau_k}, G(\theta_{k-\tau_k},\omega_{k-\tau_k},X_k)-G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)\right\rangle\mid\Fcal_{k-\tau_k}\big]\notag\\
&\leq  2D\hspace{-2pt}\left\|z_{k-\tau_k}\right\|\hspace{-1pt}(\|\theta_{k-\tau_k}\|\hspace{-2pt}+\hspace{-2pt}\|\omega_{k-\tau_k}\|\hspace{-2.5pt}+\hspace{-2.5pt}1)\big\|\Eset\big[d_{TV}(p_{k-1}(\cdot),\tilde{p}_{k-1}(\cdot)) \hspace{-2pt}+\hspace{-2pt} L\|\theta_{k-1}\hspace{-2pt}-\hspace{-2pt}\theta_{k-\tau_k}\|\hspace{-1pt}\mid\hspace{-2pt}\Fcal_{k-\tau_{k}}\big]\notag\\
&\leq  2LD\left\|z_{k-\tau_k}\right\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)\sum_{t=k-\tau_{\alpha_{k}}}^{k-1}\Eset\big[\|\theta_{t}-\theta_{k-\tau_k}\|\mid\Fcal_{k-\tau_k}\big]\notag, 
\end{align}
where the last inequality we use $d_{TV}(p_{k-\tau_k}(\cdot),\tilde{p}_{k-\tau_k}(\cdot)) = 0$. Since the operator $H$ is bounded (assumed in \eqref{assump:H_bounded}) we have
\begin{align*}
    \sum_{t=k-\tau_k+1}^{k-1} \hspace{-7pt}\|\theta_t\hspace{-2pt}-\hspace{-2pt}\theta_{k-\tau_k}\|]\hspace{-2pt}\leq\hspace{-5pt} \sum_{t=k-\tau_k+1}^{k}\sum_{t'=k-\tau_k}^{t-1} \hspace{-7pt}\|\theta_{t'+1}\hspace{-2pt}-\hspace{-2pt}\theta_{t'}\|]\hspace{-2pt}\leq \hspace{-6pt}\sum_{t=k-\tau_k+1}^{k}\sum_{t'=k-\tau_k}^{t-1}\hspace{-7pt}B\alpha_{k-\tau_k}\leq B\tau_k^2\alpha_{k-\tau_k},
\end{align*}
which we substitute into the equation above and take the expectation on both sides
\begin{align}
    T_{4}&\leq 2DBL\tau_k^2\alpha_{k-\tau_k}\mathbb{E}\big[\left\|z_{k-\tau_k}\right\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)\big].
\end{align}
On the other hand, we consider
\begin{align}
    &\left\|z_{k-\tau_k}\right\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)\notag\\
    % &\leq \left\|z_{k-\tau_k}\right\|(\|\theta_{k}\|+\|\theta_{k}-\theta_{k-\tau_k}\|+\|\omega_{k}\|+\|\omega_{k}-\omega_{k-\tau_k}\|+1)\notag\\
    &\leq \left\|z_{k-\tau_k}\right\|(\|\theta_k\|+B\tau_k\alpha_{k-\tau_k}+\|\omega_{k}\|+\|\omega_{k}-\omega_{k-\tau_k}\|+1)\notag\\
    &\leq \left\|z_{k-\tau_k}\right\|(\|\theta_k\|+\|\omega_{k}\|+\frac{1}{2}(\|\omega_k\|+\|\theta_k\|+1)+\frac{7}{6})\notag\\
    &\leq 2\left\|z_{k-\tau_k}\right\|(\|\theta_k\|+\|\omega_{k}\|+1)\leq \left\|z_{k-\tau_k}\right\|^2+(\|\theta_k\|+\|\omega_{k}\|+1)^2\notag\\
    &\leq \left\|z_{k-\tau_k}\right\|^2+3(\|\theta_k\|^2+\|\omega_{k}\|^2+1),\label{lem:Lambda_bound:eq1d1}
\end{align}
where the second inequality uses the step size condition $B\tau_k\alpha_{k-\tau_k}\leq\frac{1}{6}$ and Lemma \ref{lem:omega_k-omega_k-tau}. Using \eqref{lem:Lambda_bound:eq1d1} in the equation above, we have
\begin{align}
    T_{4}&\leq DBL\tau_k^2\alpha_{k-\tau_k}\mathbb{E}\big[\left\|z_{k-\tau_k}\right\|^2\big]+3DBL\tau_k^2\alpha_{k-\tau_k}\mathbb{E}\big[\|\theta_k\|^2+\|\omega_{k}\|^2+1\big].\label{lem:Lambda_bound:eq1d}
\end{align}
Next, we bound $T_{5}$ using Assumption \ref{assump:markov-chain}
\begin{align*}
T_{5} &=
    \Eset\Big[\mathbb{E}\big[\left\langle z_{k-\tau_k}, G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)-\mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]\right\rangle\mid\Fcal_{k-\tau_k}\big]\Big]\notag\\
    % &=\Eset\Big[\left\langle z_{k-\tau_k}, \mathbb{E}\big[G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)-\mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]\mid\Fcal_{k-\tau_k}\big]\right\rangle\Big]\notag\\
    &\leq \Eset[\|z_{k-\tau_k}\| \big\|\mathbb{E}[G(\theta_{k-\tau_k},\omega_{k-\tau_k}, \widetilde{X}_k)-\mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]\mid\Fcal_{k-\tau_k}]\big\|]\notag\\
    &\leq D\Eset[\|z_{k-\tau_k}\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)\mathbb{E}[d_{TV}(\widetilde{p}_k(\cdot),\mu_{\theta_{k-\tau_k}})\mid\Fcal_{k-\tau_k}]]\notag\\
    &\leq D\alpha_{k}\Eset[\|z_{k-\tau_k}\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)]\notag\\
    &\leq D\alpha_{k}\mathbb{E}[\|z_{k-\tau_k}\|^2\big]+3D\alpha_{k}\mathbb{E}\big[\|\theta_k\|^2+\|\omega_k\|^2+1],
    % &\leq D\|z_{k-\tau_k}\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1)m\rho^{\tau_k}.
\end{align*}
where the last inequality is due to \eqref{lem:Lambda_bound:eq1d1}. 
We next consider $T_{6}$,
\begin{align*}
    &\mathbb{E}\big[\left\langle z_{k-\tau_k}, \mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\hat{X})]\right\rangle\mid\Fcal_{k-\tau_k}\big]\notag\\
    % &= \left\langle z_{k-\tau_k}, \mathbb{E}\big[\hspace{-1pt}\mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}\hspace{-2pt}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]\hspace{-1pt}-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\hat{X})]\mid\Fcal_{k-\tau_k}\big]\right\rangle\notag\\
    &\leq \left\|z_{k-\tau_k}\right\| \left\|\mathbb{E}\big[\hspace{-1pt}\mathbb{E}_{\bar{X}\sim \mu_{\theta_{k-\tau_k}}}\hspace{-3pt}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\bar{X})]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\hat{X})]\mid\Fcal_{k-\tau_k}\big]\right\|\notag\\
    &\leq \left\|z_{k-\tau_k}\right\|D(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1) \mathbb{E}\big[d_{TV}(\mu_{\theta_k},\mu_{\theta_{k-\tau_k}})\mid\Fcal_{k-\tau_k}\big]\notag\\
    &\leq D L\left\|z_{k-\tau_k}\right\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1) \mathbb{E}[\|\theta_k-\theta_{k-\tau_k}\|\mid\Fcal_{k-\tau_k}]\notag\\
    &\leq D B L\tau_k\alpha_{k-\tau_k}\left\|z_{k-\tau_k}\right\|(\|\theta_{k-\tau_k}\|+\|\omega_{k-\tau_k}\|+1),
\end{align*}
where the third inequality uses \eqref{assump:tv_bound:eq2} in Assumption \ref{assump:tv_bound}. Again, we can employ \eqref{lem:Lambda_bound:eq1d1}
\begin{align*}
    T_{6}&\leq DBL\tau_k\alpha_{k-\tau_k}\mathbb{E}\big[\|z_{k-\tau_k}\|^2\big]+3DBL\tau_k\alpha_{k-\tau_k}\mathbb{E}\big[\|\theta_k\|^2+\|\omega_k\|^2+1\big].
\end{align*}
Finally, using the Cauchy-Schwarz inequality and the Lipschitz continuity of $G$,
\begin{align*}
    &T_{7}
    \leq\mathbb{E}\big[\left\|z_{k-\tau_k}\right\|\left\| \mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_{k-\tau_k},\omega_{k-\tau_k},\hat{X})-G(\theta_{k},\omega_{k},\hat{X})]\right\|\big]\notag\\
    &\leq L\mathbb{E}\big[\left\|z_{k-\tau_k}\right\|\left(\|\theta_k-\theta_{k-\tau_k}\|+\|\omega_k-\omega_{k-\tau_k}\|\right)\big]\notag\\
    &\leq\mathbb{E}\big[\frac{L (B\hspace{-2pt}+\hspace{-2pt}3D)\tau_k\beta_{k-\tau_k}}{2}\|z_{k-\tau_k}\|^2\hspace{-2pt}+\hspace{-2pt}\frac{9L D\tau_k\beta_{k-\tau_k}}{2}\|\omega_k\|^2\hspace{-2pt}+\hspace{-2pt}\|\theta_{k}\|^2\big]+\frac{L (B\hspace{-2pt}+\hspace{-2pt}9D)\tau_k\beta_{k-\tau_k}}{2},
    % \label{lem:Lambda_bound:eq1f}
\end{align*}
where the derivation of the last inequality is identical to that of $T_{3}$. 
Finally, plugging the bound on $T_1$-$T_7$
% \eqref{lem:Lambda_bound:eq1a}--\eqref{lem:Lambda_bound:eq1f}
in \eqref{lem:Lambda_bound:Eq0} and simplifying the terms using the relations $\alpha_k\leq\beta_k$, $\tau_k\geq 1$ leads to the claimed result.


==> header_1.tex <==
% CALLIGRAPHIC AND BOLD SYMBOLS 
\newcommand{\Aset}{\mathbb{A}}
\newcommand{\Bset}{\mathbb{B}}
\newcommand{\Cset}{\mathbb{C}}
\newcommand{\Dset}{\mathbb{D}}
\newcommand{\Eset}{\mathbb{E}}
\newcommand{\Fset}{\mathbb{F}}
\newcommand{\Gset}{\mathbb{G}}
\newcommand{\Hset}{\mathbb{H}}
\newcommand{\Iset}{\mathbb{I}}
\newcommand{\Jset}{\mathbb{J}}
\newcommand{\Kset}{\mathbb{K}}
\newcommand{\Lset}{\mathbb{L}}
\newcommand{\Mset}{\mathbb{M}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\Oset}{\mathbb{O}}
\newcommand{\Pset}{\mathbb{P}}
\newcommand{\Qset}{\mathbb{Q}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Sset}{\mathbb{S}}
\newcommand{\Tset}{\mathbb{T}}
\newcommand{\Uset}{\mathbb{U}}
\newcommand{\Vset}{\mathbb{V}}
\newcommand{\Wset}{\mathbb{W}}
\newcommand{\Xset}{\mathbb{X}}
\newcommand{\Yset}{\mathbb{Y}}
\newcommand{\Zset}{\mathbb{Z}}


\newcommand{\Acal}{{\cal A}}
\newcommand{\Bcal}{{\cal B}}
\newcommand{\Ccal}{{\cal C}}
\newcommand{\Dcal}{{\cal D}}
\newcommand{\Ecal}{{\cal E}}
\newcommand{\Fcal}{{\cal F}}
\newcommand{\Gcal}{{\cal G}}
\newcommand{\Hcal}{{\cal H}}
\newcommand{\Ical}{{\cal I}}
\newcommand{\Jcal}{{\cal J}}
\newcommand{\Kcal}{{\cal K}}
\newcommand{\Lcal}{{\cal L}}
\newcommand{\Mcal}{{\cal M}}
\newcommand{\Ncal}{{\cal N}}
\newcommand{\Ocal}{{\cal O}}
\newcommand{\Pcal}{{\cal P}}
\newcommand{\Qcal}{{\cal Q}}
\newcommand{\Rcal}{{\cal R}}
\newcommand{\Scal}{{\cal S}}
\newcommand{\Tcal}{{\cal T}}
\newcommand{\Ucal}{{\cal U}}
\newcommand{\Vcal}{{\cal V}}
\newcommand{\Wcal}{{\cal W}}
\newcommand{\Xcal}{{\cal X}}
\newcommand{\Ycal}{{\cal Y}}
\newcommand{\Zcal}{{\cal Z}}

\newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\Bfrak}{\mathfrak{B}}
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\Dfrak}{\mathfrak{D}}
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\Gfrak}{\mathfrak{G}}
\newcommand{\Hfrak}{\mathfrak{H}}
\newcommand{\Ifrak}{\mathfrak{I}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\Kfrak}{\mathfrak{K}}
\newcommand{\Lfrak}{\mathfrak{L}}
\newcommand{\Mfrak}{\mathfrak{M}}
\newcommand{\Nfrak}{\mathfrak{N}}
\newcommand{\Ofrak}{\mathfrak{O}}
\newcommand{\Pfrak}{\mathfrak{P}}
\newcommand{\Qfrak}{\mathfrak{Q}}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Sfrak}{\mathfrak{S}}
\newcommand{\Tfrak}{\mathfrak{T}}
\newcommand{\Ufrak}{\mathfrak{U}}
\newcommand{\Vfrak}{\mathfrak{V}}
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\Xfrak}{\mathfrak{X}}
\newcommand{\Yfrak}{\mathfrak{Y}}
\newcommand{\Zfrak}{\mathfrak{Z}}

\newcommand{\Asf}{\sf{A}}
\newcommand{\Bsf}{\sf{B}}
\newcommand{\Csf}{\sf{C}}
\newcommand{\Dsf}{\sf{D}}
\newcommand{\Esf}{\sf{E}}
\newcommand{\Fsf}{\sf{F}}
\newcommand{\Gsf}{\sf{G}}
\newcommand{\Hsf}{\sf{H}}
\newcommand{\Isf}{\sf{I}}
\newcommand{\Jsf}{\sf{J}}
\newcommand{\Ksf}{\sf{K}}
\newcommand{\Lsf}{\sf{L}}
\newcommand{\Msf}{\sf{M}}
\newcommand{\Nsf}{\sf{N}}
\newcommand{\Osf}{\sf{O}}
\newcommand{\Psf}{\sf{P}}
\newcommand{\Qsf}{\sf{Q}}
\newcommand{\Rsf}{\sf{R}}
\newcommand{\Ssf}{\sf{S}}
\newcommand{\Tsf}{\sf{T}}
\newcommand{\Usf}{\sf{U}}
\newcommand{\Vsf}{\sf{V}}
\newcommand{\Wsf}{\sf{W}}
\newcommand{\Xsf}{\sf{X}}
\newcommand{\Ysf}{\sf{Y}}


\newcommand{\Abf}{{\bf A}}
\newcommand{\Bbf}{{\bf B}}
\newcommand{\Cbf}{{\bf C}}
\newcommand{\Dbf}{{\bf D}}
\newcommand{\Ebf}{{\bf E}}
\newcommand{\Fbf}{{\bf F}}
\newcommand{\Gbf}{{\bf G}}
\newcommand{\Hbf}{{\bf H}}
\newcommand{\Ibf}{{\bf I}}
\newcommand{\Jbf}{{\bf J}}
\newcommand{\Kbf}{{\bf K}}
\newcommand{\Lbf}{{\bf L}}
\newcommand{\Mbf}{{\bf M}}
\newcommand{\Nbf}{{\bf N}}
\newcommand{\Obf}{{\bf O}}
\newcommand{\Pbf}{{\bf P}}
\newcommand{\Qbf}{{\bf Q}}
\newcommand{\Rbf}{{\bf R}}
\newcommand{\Sbf}{{\bf S}}
\newcommand{\Tbf}{{\bf T}}
\newcommand{\Ubf}{{\bf U}}
\newcommand{\Vbf}{{\bf V}}
\newcommand{\Wbf}{{\bf W}}
\newcommand{\Xbf}{{\bf X}}
\newcommand{\Ybf}{{\bf Y}}
\newcommand{\Zbf}{{\bf Z}}



\newcommand{\Xbarbf}{{\bar{\Xbf}}}




% ---------  lower case  --------------
\newcommand{\abf}{{\bf a}}
\newcommand{\bbf}{{\bf b}}
\newcommand{\cbf}{{\bf c}}
\newcommand{\dbf}{{\bf d}}
\newcommand{\ebf}{{\bf e}}
\newcommand{\fbf}{{\bf f}}
\newcommand{\gbf}{{\bf g}}
\newcommand{\hbf}{{\bf h}}
\newcommand{\ibf}{{\bf i}}
\newcommand{\jbf}{{\bf j}}
\newcommand{\kbf}{{\bf k}}
\newcommand{\lbf}{{\bf \ell}}
\newcommand{\mbf}{{\bf m}}
\newcommand{\nbf}{{\bf n}}
\newcommand{\obf}{{\bf o}}
\newcommand{\pbf}{{\bf p}}
\newcommand{\qbf}{{\bf q}}
\newcommand{\rbf}{{\bf r}}
\newcommand{\sbf}{{\bf s}}
\newcommand{\tbf}{{\bf t}}
\newcommand{\ubf}{{\bf u}}
\newcommand{\vbf}{{\bf v}}
\newcommand{\wbf}{{\bf w}}
\newcommand{\xbf}{{\bf x}}
\newcommand{\ybf}{{\bf y}}
\newcommand{\zbf}{{\bf z}}


\newcommand{\xhatbf}{{\hat{\xbf}}}
\newcommand{\ehatbf}{{\hat{\ebf}}}

\newcommand{\xdagbf}{{\xbf^{\dagger}}}
\newcommand{\ydagbf}{{\ybf^{\dagger}}}

\newcommand{\xibarbf}{{\bar{\xibf}}}
\newcommand{\btheta}{{\bar{\theta}}}

\newcommand{\ebarbf}{{\bar{\ebf}}}
\newcommand{\qbarbf}{{\bar{\qbf}}}
\newcommand{\xbarbf}{{\bar{\xbf}}}
\newcommand{\vbarbf}{{\bar{\vbf}}}
\newcommand{\rbarbf}{{\bar{\rbf}}}
\newcommand{\zbarbf}{{\bar{\zbf}}}

\newcommand{\tmin}{\tau_{\min}}
\newcommand{\tmax}{\tau_{\max}}
\newcommand{\tbar}{\bar{\tau}}
\newcommand{\tbbf}{\boldsymbol{\tbar}}


\newcommand{\xdot}{\dot{x}}
\newcommand{\ydot}{\dot{y}}

\newcommand{\1}{{\mathbf{1}}}
\newcommand{\bld}{{\boldsymbol{\lambda}}}
\newcommand{\Phibf}{{\boldsymbol{\phi}}}
\newcommand{\phibf}{{\boldsymbol{\Phi}}}
\newcommand{\xibf}{{\boldsymbol{\xi}}}
\newcommand{\Xibf}{{\boldsymbol{\Xi}}}


\newcommand{\omegabf}{{\boldsymbol{\omega}}}
\newcommand{\epsilonbf}{{\boldsymbol{\epsilon}}}


%------  bar  --------- 
\newcommand{\cbar}{{\bar{c}}}
\newcommand{\ebar}{{\bar{e}}}
\newcommand{\xbar}{{\bar{x}}}
\newcommand{\ybar}{{\bar{y}}}
\newcommand{\gbar}{{\bar{g}}}
\newcommand{\rbar}{{\bar{r}}}
\newcommand{\qbar}{{\bar{q}}}
\newcommand{\vbar}{{\bar{v}}}
\newcommand{\zbar}{{\bar{z}}}



\newcommand{\phibar}{{\bar{\phi}}}
\newcommand{\xibar}{{\bar{\xi}}}


\newcommand{\xhat}{{\hat{x}}}
\newcommand{\ehat}{{\hat{e}}}


\newcommand{\xdag}{{x^\dagger}}
\newcommand{\ydag}{{y^\dagger}}



\newcommand{\zetabf}{{\mathbf{\zeta}}}



% MISCELLANEOUS
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\Hinf}{{\cal H}_\infty}
\newcommand{\Htwo}{{\cal H}_2}
\newcommand{\bone}{\mathbf{1}}

\renewcommand{\arraystretch}{1.1}

\newcommand{\wtilde}[1]{\widetilde{#1}}

\renewcommand{\v}[1]{{\mathbf{#1}}}
\newcommand{\ve}{\varepsilon}
\newcommand{\sgn}{\text{sgn }}
\newcommand{\ii}{\mathbf{i}}




%\theoremstyle{plain}
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
% \theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{prob}{Problem}
\newtheorem{assump}{Assumption}
%\newtheorem{algorithm}{Algorithm}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}
%\newtheorem*{remark}{Remark}
%\newtheorem{example}{Example}
%\newtheorem{notation}{\bf{Notation}}


\newcommand{\addcite}{{\textcolor{red}{(addcite) }}}

\newcommand{\redline}{\raisebox{2pt}{\tikz{\draw[-,red,solid,line width = 1.5pt](0,0) -- (6mm,0);}}}
\newcommand{\blueline}{\raisebox{2pt}{\tikz{\draw[-,blue,solid,line width = 1.5pt](0,0) -- (6mm,0);}}}
\newcommand{\greenline}{\raisebox{2pt}{\tikz{\draw[-,green,solid,line width = 1.5pt](0,0) -- (6mm,0);}}}

\newcommand{\blackline}{\raisebox{2pt}{\tikz{\draw[-,black,solid,line width = 1.5pt](0,0) -- (6mm,0);}}}

\newcommand{\tdoan}[1]{{\color{red}\bf [tdoan: #1]}}


==> old_files/Dec1_2022_combinelambda/Analysis_Assumptions.tex <==
\section{Technical Assumptions}
\label{sec:assumptions}
In this section, we present the main technical assumptions important in our later analysis. We first consider the smoothness assumption of $H$ and $G$ and the boundedness condition of $H$. 
\begin{assump}\label{assump:HG_smooth}
There exists a constant $L > 0$ such that for all $\theta_{1},\theta_{2}\in\Rset^{d},$ $\omega_{1},\omega_{2}\in\Rset^{r}$, and $X\in\Xcal$ 
\begin{align}
    &\left\|H(\theta_1,\omega_1,X)-H(\theta_2,\omega_2,X)\right\| \leq L\left(\|\theta_1-\theta_2\|+\|\omega_1-\omega_2\|\right),\notag\\
    &\left\|G(\theta_1,\omega_1,X)-G(\theta_2,\omega_2,X)\right\| \leq L\left(\|\theta_1-\theta_2\|+\|\omega_1-\omega_2\|\right).\label{assump:HG_smooth:ineq}
\end{align}
% In addition, there exists a constant $B>0$ such that 
% \begin{align}
% \|H(\theta,\omega,X)\| \leq B,\quad \forall \theta\in\Rset^{d}, \omega\in\Rset^{r},X\in\Xcal.    \label{assump:H_bounded}
% \end{align}
\end{assump}
We also assume the smoothness of the objective function $f$. 
\begin{assump}\label{assump:f_smooth}
There exists a constant $L>0$ such that for all $\theta_{1},\theta_{2}\in\Rset^{d}$
\begin{align}
    % &\left\|\nabla f(\theta)\right\| \leq B, \quad \forall \theta \in \mathbb{R}^{d}\\
    % \text{and   }& 
    \left\|\nabla f(\theta_1)-\nabla f(\theta_2)\right\| \leq L\|\theta_1-\theta_2\|.\label{assump:f_smooth:ineq}
    % , \quad \forall\theta_1,\theta_2 \in \mathbb{R}^{d}
\end{align}
\end{assump}
Assumptions \ref{assump:HG_smooth} and \ref{assump:f_smooth} are common in the literature of stochastic approximation \cite{karmakar2018two,doan2021finite} and hold in the context of actor-critic methods, which we will verify in Section \ref{sec:applications}. Next, we assume that the operator $G$ is strongly monotone in expectation at its root (which we have assumed is unique). 


\begin{assump}\label{assump:stronglymonotone_G}
There exists a constant $\lambda_G>0$ such that
\begin{align*}
    \left\langle \Eset_{X\sim\mu_{\theta}}[G(\theta,\omega,X)],\omega-\omega^{\star}(\theta)\right\rangle \leq -\lambda_G\|\omega-\omega^{\star}(\theta)\|^2,\quad \forall \theta \in \mathbb{R}^{d},\omega \in \mathbb{R}^{r}.
\end{align*}
\end{assump}
This assumption is often made in the existing literature on two-time-scale stochastic approximation \cite{hong2020two,doan2021finite} and is a sufficient condition to guarantee the fast convergence of the auxiliary variable iterate.
{\color{red} This assumption essentially states that $G$ in expectation behaves similarly to the gradient of a strongly convex function, though it may not even be a gradient mapping.}
% On the other hand, the existence and uniqueness of $\omega^{\star}(\theta)$ can also be guaranteed if we assume that $G$ is contractive. 
% Our results given in the next section are also applicable under this condition.  
We will verify that Assumption \ref{assump:stronglymonotone_G} (or an equivalent contractive condition) holds in the actor-critic methods discussed in Section \ref{sec:applications}. 

In addition, we assume that the solution $\omega^{\star}(\cdot)$ is $L$-Lipschitz continuous with respect to $\theta$ as follows.    
\begin{assump}\label{assump:Lipschitz_omega}
There exists a constant $L,B>0$ such that
\begin{align*}
    \left\|\omega^{\star}(\theta)-\omega^{\star}(\theta')\right\| \leq L\|\theta-\theta'\|, \quad \left\|\omega^{\star}(\theta)\right\|\leq B, \quad \forall \theta,\theta' \in \mathbb{R}^{d}.
\end{align*}
\end{assump}
Note that we use the same constant $L$ in the three assumptions above for the convenience of notation. 

Given two probability distributions $\mu_1$ and $\mu_2$ over the space $\Xcal$, their total variation (TV) distance is defined as
\begin{equation}
    \label{eq:TV_def}
    d_{\text{TV}}(\mu_1,\mu_2)=\frac{1}{2} \sup _{\nu: \Xcal \rightarrow[-1,1]}\left|\int \nu d \mu_1-\int \nu d \mu_2\right|.
\end{equation}
The definition of the mixing time of a Markov chain $\{X_{k}\}$ is given as follows.
\begin{definition}
    \label{def:mixing_time}
    Consider the Markov chain $\{X_k^{\theta}\}$ generated according to $X_k^{\theta}\sim\Pcal(\cdot\mid X_{k-1}^{\theta},\theta)$, and let $\mu_{\theta}$ be its stationary distribution.  For any $\alpha>0$, the mixing time of the chain $\{X_k^{\theta}\}$ corresponding to $\alpha$ is defined as
    \[
        \tau_{\theta}(\alpha) = \min\{k\in\mathbb{N}:\sup_{X\in\Xcal}d_{\text{TV}}(P(X_k^{\theta}=\cdot\mid X_0^{\theta}=X),\mu_{\theta}(\cdot))\leq \alpha\}.
    \]
\end{definition}
The mixing time $\tau_{\theta}(\alpha)$ essentially measures the time needed for the Markov chain $\{X_{k}^{\theta}\}$ to approach its stationary distribution \cite{LevinPeresWilmer2006}. We next consider the following important assumption that guarantees that the Markov chain induced by any static $\theta$ ``mixes'' geometrically.
\begin{assump}
    \label{assump:markov-chain}
    Given any $\theta$, the Markov chain $\{X_{k}\}$ generated by $\Pcal(\cdot\mid\cdot,\theta)$ has a unique stationary distribution $\mu_{\theta}$ and is uniformly geometrically ergodic. In other words, there exist constants $m>0$ and $\rho\in (0,1)$ independent of $\theta$ such that
    \begin{equation*}
        \sup_{X\in\Xcal}d_{\text{TV}}(P(X_k=\cdot\,|X_0=X,\,\theta),\mu_{\theta}(\cdot))\leq m\rho^k \text{ for all } \theta\in\mathbb{R}^d\text{~and }k\geq 0. 
    \end{equation*}
\end{assump}
Denoting $\tau(\alpha)\triangleq\sup_{\theta\in\mathbb{R}^d}\tau_{\theta}(\alpha)$, this assumption implies that there exists a positive constant $C$ depending only on $\rho$ and $m$ such that 
\begin{equation}
    \tau(\alpha) \leq C\log\left(1/\alpha\right).\label{assump:mixing:tau}
\end{equation} 
Assumption \ref{assump:markov-chain} is again standard in the analysis of algorithms under time-varying Markovian samples \cite{zou2019finite,wu2020finite}. 

We also consider the following assumption on the ensemble of transition kernels.
% \begin{assump}
%     \label{assump:tv_bound}
%     Given $\theta,\hat{\theta}\in\mathbb{R}^d$ and $X,\hat{X}\in\Xcal$, let $X'\sim \Pcal(\cdot\mid X,\theta)$ and $\hat{X}'\sim \Pcal(\cdot\mid\hat{X},\theta')$. Then there exists a constant $L>0$ 
%     \begin{align}
%         &d_{\text{TV}}(P(X'=\cdot), P(\hat{X}'=\cdot)) \leq d_{\text{TV}}(P(X=\cdot), P(\hat{X}=\cdot)) + L\|\theta-\hat{\theta}\|.
%         \label{assump:tv_bound:eq1}
%     \end{align}
%     In addition, we assume that 
%     \begin{align}
%         d_{\text{TV}}(\mu_{\theta}, \mu_{\hat{\theta}})\leq L\|\theta-\hat{\theta}\|.
%         \label{assump:tv_bound:eq2}
%     \end{align}
% \end{assump}
{\color{red}
\begin{assump}
    \label{assump:tv_bound}
    Given two distributions $d,\hat{d}$ over $\Xcal$ and control parameters $\theta,\hat{\theta}\in\mathbb{R}^d$, we draw the samples according to
    $X\sim d, X'\sim\Pcal(\cdot\mid X,\theta)$ and $\hat{X}\sim\hat{d},\hat{X}'\sim \Pcal(\cdot\mid\hat{X},\hat{\theta})$.
    There exists a constant $L>0$ 
    \begin{align}
        &d_{\text{TV}}(P(X'=\cdot), P(\hat{X}'=\cdot)) \leq d_{\text{TV}}(d, \hat{d}) + L\|\theta-\hat{\theta}\|.
        \label{assump:tv_bound:eq1}
    \end{align}
    In addition, we assume that the stationary distribution is Lipschitz in the control parameter
    \begin{align}
        d_{\text{TV}}(\mu_{\theta}, \mu_{\hat{\theta}})\leq L\|\theta-\hat{\theta}\|.
        \label{assump:tv_bound:eq2}
    \end{align}
\end{assump}
}
This assumption amounts to a regularity condition on the transition probability matrix $\Pcal(\cdot\mid\cdot,\theta)$ as a function of $\theta$, and has been shown to hold in the reinforcement learning setting (see, for example, \cite[Lemma A1]{wu2020finite}). Without loss of generality, we use the same constant $L$ as in Assumptions \ref{assump:HG_smooth}--\ref{assump:Lipschitz_omega} and assume $B\geq 1$. We define\vspace{-2pt}
\begin{equation}
D = \max\{L+\max_{X\in\Xcal}\|G(0,0,X)\|,\|\omega^*(0)\|,B\},  
\label{notation:D}
\end{equation}
which is a finite constant since $\Xcal$ is compact. A simple consequence of \eqref{notation:D} and Assumption \ref{assump:HG_smooth} is that for all $\theta\in\mathbb{R}^d,\omega\in\mathbb{R}^r,X\in\Xcal$
\begin{gather}
    \|G(\theta,\omega,X)\|\leq D(\|\theta\|+\|\omega\|+1),\quad\text{and}\quad
    \|\omega^{\star}(\theta)\|\leq D(\|\theta\|+1).\label{eq:G_affinelybounded_D}
\end{gather}
Finally, we assume the optimal solution set $\{\theta^{\star}\hspace{-2pt}:f(\theta^{\star})\leq f(\theta),\,\forall \theta\in\mathbb{R}^{d}\}$ is non-empty.


==> old_files/Dec1_2022_combinelambda/Analysis_Theorems.tex <==

\section{Main Results}\label{sec:main_results}
In Section~\ref{subsec:main_theorems}, we present the main results of this paper, which are the finite-time convergence of Algorithm \ref{Alg:two-time-scale-SGD} under different function structure. Then, we briefly explain the main technical challenges and the complex coupling of the decision variable, auxiliary variable, and time-varying Markovian samples in Section \ref{subsec:tech_challenges}. 
% We then state the convergence of the auxiliary variable in Section \ref{subsec:conv_auxiliary}, which is an important step towards deriving the convergence of the decision variable.
In Section \ref{sec:lyapunov_lemma}, we introduce an important lemma that performs Lyapunov analysis on a coupled dynamical system of two inequalities. This lemma is a unified tool to analyze our algorithm under different function structures and may be of independent interest in the study of the finite-time performance of multiple-time-scale dynamical systems apart from those considered in this paper. Finally, we prove the theorem under the P\L~condition in Section~\ref{sec:proof_mainresults}. Strongly convex and general non-convex functions can be treated with similar analytical techniques, and the full details of their analyses can be found in the companion paper \cite{zeng2021two}.


\subsection{Finite-Time Complexity of Two-Time-Scale SGD}\label{subsec:main_theorems}
This subsection establishes the finite-time complexity of the two-time-scale SGD algorithm under four structural properties of the objective function, namely, strong convexity,
non-convexity with the P\L~condition, and general non-convexity. Our results are derived under the assumptions introduced in Section \ref{sec:assumptions}, which we assume always hold in the rest of this paper.


The convergence of Algorithm \ref{Alg:two-time-scale-SGD} relies on $\alpha_k,\beta_k\rightarrow 0$ with reasonable rates. As mentioned in Section \ref{sec:two-time-scale-SGD}, $\alpha_{k}$ needs to be much smaller than $\beta_{k}$ to approximate the nested-loop algorithm where multiples auxiliary variable updates are performed for each decision variable update. Therefore, we consider the following choices of step sizes\looseness=-1
\begin{align}
    \alpha_k = \frac{\alpha_0}{(k+1)^{a}}, \quad \beta_k = \frac{\beta_0}{(k+1)^{b}},\quad\forall k\geq 0,\label{stepsizes}
\end{align}
where $a,b,\alpha_0,\beta_0$ are some constants satisfying $0 < b\leq a\leq 1$ and $0< \alpha_0 \leq  \beta_0$. 
Given $\alpha_{k}$, recall from Definition \ref{def:mixing_time} that  $\tau(\alpha_{k})$ is the mixing time associated with $\alpha_{k}$. In the sequel, for convenience we denote $\tau_{k}\triangleq\tau(\alpha_k)$.
Since $\tau_{k} \leq C\log((k+1)^{a}/\alpha_0)$ (from \eqref{assump:mixing:tau}), we have
$\lim_{k\rightarrow\infty}\alpha_{k}\tau_{k}^2 = \lim_{k\rightarrow\infty}\beta_{k}\tau_{k}^2 = 0$.
This implies that there exists a positive integer $\Kcal$ such that
\begin{align}
    \beta_{k-\tau_k}\tau_k^2\leq\min\Big\{1,\frac{1}{6LB},\frac{\lambda_G}{22C_1+32D^2},\frac{\lambda_f}{2C_2},\frac{\lambda_f^2 \lambda_G}{32L^2 C_2}\Big\},\quad\forall k\geq\Kcal,\label{notation:Kcal}
\end{align}
where $C_1$ and $C_2$ are positive constants defined as 
\begin{align}
C_1 &= 18D^2+20LDB,\,\,C_2=(4D^2+1)(4C_1+32D^2)+\frac{2L^2 B^2}{\lambda_G}+2L^2 B^2.
\label{notation:constant_C}   
\end{align}
% \begin{align}
% \begin{aligned}
% C_1 &= 18D^2+7LDB+9LD+LB+3D,\\
% C_2&=(4D^2+1)(4C_1+32D^2)+\frac{2L^2 B^2}{\lambda_G}+2L^2 B^2,\\ 
% C_3&=4\left(BL^2+B^2 L^2+B^2 L+B+B^2+L^2\right),\\
% C_4&=2C_2\|\theta^{\star}\|^2 + C_2 + 3C_3+B^2,\\
% C_5&=4B^3 L+4B^2L+2B^2 L^2+2B^2\\
% C_6&=(12C_5+6L B^2)\frac{\alpha_0^2}{c_{\tau}}+\frac{48C_2 L^2}{\lambda_G} (\|\theta_0\|^2+B^2 \alpha_0^2+1)\frac{\alpha_0\beta_0}{c_{\tau}}+\frac{48L^4 B^2 \alpha_0^3}{\lambda_G^2 \beta_0^2}\\
% C_7&=(2B^2\hspace{-2pt}+\hspace{-2pt}1)(4C_1\hspace{-2pt}+\hspace{-2pt}4D^2)\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2}{\lambda_G}\hspace{-2pt}+\hspace{-2pt}2L^2 B^2\\
% C_8&=\frac{\alpha_0^2 (2C_5\hspace{-2pt}+\hspace{-2pt}L B^2)}{2c_{\tau}}\hspace{-2pt}+\hspace{-2pt}\frac{2L^4 B^2 \alpha_0^3}{\lambda_G \beta_0^2}\hspace{-2pt}+\hspace{-2pt}\frac{L^2 \alpha_0\beta_0 C_7}{c_{\tau}\lambda_G}.
% \end{aligned}\label{notation:constant_C}   
% \end{align}
In addition, there exists a constant $c_{\tau}\in(0,1)$ such that for any $k>\tau_k$ we have
\begin{align}
    \tau_k\leq(1-c_{\tau})k+(1-c_{\tau}), \quad\text{and}\quad c_{\tau}(k+1)\leq k-\tau_k+1\leq k+1.
\end{align}

We carefully come up with the constants and conditions in \eqref{notation:Kcal} and \eqref{notation:constant_C} to prevent an excessively large step size from destroying the stability of the updates. We note that $\Kcal$ is a constant that only depends on the quantities involved in the step sizes in \eqref{stepsizes}.


\subsubsection{Strong Convexity} We consider the following assumption on function $f$. 

\begin{assump}\label{assump:sc}
The function $f$ is strongly convex with constant $\lambda_{f}$
\begin{align}
    f(y) \geq f(x)+\langle\nabla f(x),y-x\rangle+\frac{\lambda_f}{2}\|y-x\|^{2}, \quad \forall x,y\in\mathbb{R}^d.\label{assump:sc:ineq}
\end{align}
\end{assump}
Our first main result shows that when $f$ is strongly convex, the iterates of Algorithm~\ref{Alg:two-time-scale-SGD} converge to the optimal solution at a rate $\widetilde{\Ocal}(k^{-2/3})$ up to a logarithm factor.
\begin{thm}[Strongly Convex]
Suppose that Assumption \ref{assump:sc} holds.
Let the step size sequences $\{\alpha_k\}$ and $\{\beta_k\}$ satisfy \eqref{stepsizes} with
\begin{align*}
a=1,\quad b=2/3,\quad \alpha_0\geq \frac{4}{\lambda_f},\quad\text{and}\quad \frac{\alpha_0}{\beta_0}\leq\frac{\lambda_G}{2\lambda_f}\cdot
\end{align*}
Then for all $k\geq \Kcal$ where $\Kcal$ is defined in \eqref{notation:Kcal},
% (again, we note that $\Kcal$ is a constant depending only on $a,b,\alpha_0,\beta_0$ and the structures of the function $f$),
we have
\begin{align*}
    \mathbb{E}\left[\|\theta_k-\theta^{\star}\|^2\right]
    &\leq \frac{\Kcal+1}{k+1}\left(\mathbb{E}\left[\|\theta_{\Kcal}-\theta^{\star}\|^2\right]+\frac{4 L^{2} \alpha_0}{\lambda_{G} \lambda_{f} \beta_0}\mathbb{E}[\|\omega_{\Kcal}-\omega^{\star}(\theta_{\Kcal})\|^2]\right)\notag\\
    &\hspace{-43pt}+\frac{C^2\log^2((k+1)/\alpha_0)}{3(k+1)^{2/3}}\left((6C_2+2B^2+\frac{8L^2 C_2}{\lambda_G\lambda_f}(2\|\theta^{\star}\|^2+1))\frac{\alpha_0\beta_0}{c_{\tau}}+\frac{16L^4 B^2 \alpha_0^3}{\lambda_G^2\lambda_f \beta_0^2}\right).
    % \label{thm:convergence_decision_sc:ineq}
\end{align*}
\label{thm:convergence_decision_sc}
\end{thm}
% \begin{remark}
% Then the iterates $\theta_k$ converge to the unique optimal solution $\theta^{\star}$ at a rate of $\Ocal((k+1)^{-2/3})$ under the choice of step size $a=1$ and $b=2/3$. Compared with the standard SGD where a convergence rate of $\Ocal((k+1)^{-1})$ is achieved for strongly convex functions, the two-time-scale algorithm is slower by $\Ocal((k+1)^{1/3})$ due to the online update of the auxiliary variable.

We note that the rate in Theorem~\ref{thm:convergence_decision_sc} is similar to the one in two-time-scale SA studied in \cite{doan2021finite}. However, while \cite{doan2021finite} considers samples generated by a fixed Markov chain, the samples in our algorithm are generated by a time-varying Markov process parameterized by the decision variable. 
% \end{remark}


\subsubsection{Non-Convexity under P\L~Condition} 
We also study the convergence of Algorithm \ref{Alg:two-time-scale-SGD} under the following condition.
\begin{assump}\label{assump:PL_condition}
There exists a constant $\lambda_f>0$ such that\footnote{We slightly overload the notation and use the same constant for the P\L~condition and the strong convexity in Assumption \ref{assump:sc}.}
\[\frac{1}{2}\|\nabla f(x)\|^2 \geq \lambda_f \left(f(x)-f^{\star}\right), \quad \forall x\in\mathbb{R}^d.\]
\end{assump}
This is known as the P\L~condition and is introduced in \cite{polyak1987introduction,lojasiewicz1963topological}. The P\L~condition does not imply convexity, but guarantees the linear convergence of the objective function value when gradient descent is applied to solve a non-convex optimization problem \cite{karimi2016linear}, which resembles the convergence rate of gradient descent for strongly convex functions. Recently, this condition has been observed to hold in many important practical problems such as supervised learning with an over-parametrized neural network \cite{liu2020toward} and the linear quadratic regulator in optimal control \cite{fazel2018global,yang2019global}. 

Under the P\L~condition, we show that $f(\theta_k)$ converges to the optimal function value $f^{\star}$ with rate $\widetilde{\Ocal}(k^{-2/3})$. This is the same rate as in the case of strongly convex $f$. However, in this case the convergence is measured in the function value, whereas under strong convexity the iterates $\theta_k$ converge to the unique global minimizer.



\begin{thm}[P\L~Condition]\label{thm:convergence_decision_pl}
Suppose the function $f$ satisfies Assumption~\ref{assump:PL_condition}.
In addition, we assume that the stochastic gradient is bounded, i.e. there exists a constant $B>0$ such that \footnote{Again, for the convenience of notation, we use the same constant $B$ as in Assumption~\ref{assump:Lipschitz_omega}.}
\begin{align}
\|H(\theta,\omega,X)\| \leq B,\quad \forall \theta\in\Rset^{d}, \omega\in\Rset^{r},X\in\Xcal.    \label{assump:H_bounded}
\end{align}
Let the step size sequences $\{\alpha_k\}$ and $\{\beta_k\}$ satisfy \eqref{stepsizes} with
\begin{align*}
    a=1,\quad b=2/3,\quad\alpha_0\geq \max\{1,\frac{2}{\lambda_f}\},\quad\text{and}\quad\frac{\alpha_0}{\beta_0}\leq\frac{\lambda_G}{4\lambda_f}.
\end{align*}
Then for all $k\geq \Kcal$ where $\Kcal$ is defined in \eqref{notation:Kcal}, we have
\begin{align*}
    \mathbb{E}\left[f(\theta_{k})\hspace{-2pt}-\hspace{-2pt}f^{\star}\right]&\hspace{-3pt}\leq\hspace{-3pt} \frac{\Kcal+1}{k+1}\hspace{-2pt}\left(\hspace{-2pt}\mathbb{E}\left[f(\theta_{\Kcal})\hspace{-2pt}-\hspace{-2pt}f^{\star}\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^{2} \alpha_0}{\lambda_{G} \beta_0}\mathbb{E}[\|\omega_{\Kcal}-\omega^{\star}(\theta_{\Kcal})\|^2]\hspace{-2pt}\right)\hspace{-2pt}+\hspace{-2pt}\frac{2C^2 C_3\log^4(k\hspace{-2pt}+\hspace{-2pt}1)}{3(k+1)^{2/3}},
\end{align*}
where $C_3=\frac{150L^2B^3\alpha_0^2}{c_{\tau}}+\frac{48L^2 C_2}{\lambda_G} (\|\theta_0\|^2+B^2 \alpha_0^2+1)\frac{\alpha_0\beta_0}{c_{\tau}}+\frac{48L^4 B^2 \alpha_0^3}{\lambda_G^2 \beta_0^2}$.
\end{thm}


\subsubsection{Non-Convexity} 
Finally, we study the case where the objective function $f$ is non-convex and smooth. In general, we cannot find an optimal solution and may only reach a stationary point. Measuring the convergence in $\|\nabla f(\theta_k)\|^2$, the squared norm of the gradient, we show a convergence rate of $\widetilde{\Ocal}(k^{-2/5})$.

Analyzing the convergence without any convexity or P\L~condition is more challenging, and we need to make the following assumption that ensures stability, which replaces \eqref{assump:HG_smooth:ineq} in Assumption \ref{assump:HG_smooth}.

\begin{assump}\label{assump:HG_smooth_nonconvex}
There exists a constant $L > 0$ such that
\begin{align*}
    \left\|G(\theta_1,\omega_1,X)-G(\theta_2,\omega_2,X)\right\| \leq L(\|\omega_1-\omega_2\|+1),\forall \theta_{1},\theta_{2}\in\mathbb{R}^d,\omega_{1},\omega_{2}\in\mathbb{R}^r,X\in\Xcal.
\end{align*}
\end{assump}
We note that this assumption holds in the actor-critic algorithms we discuss in Section \ref{sec:applications} where $G$ does not depend on $\theta$, as well as in problems where $G$ is bounded in $\theta$.

% \tdoan{You should provide variants of Proposition $1$ and Lemma 3,5,6 when $H,G$ are bounded. It should not be long, basically copy from others.}


\begin{thm}[Non-convex]\label{thm:convergence_decision_nonconvex}
% Choose $a=3/5$ and $b=2/5$. 
Let the step size $\{\alpha_k\}$ and $\{\beta_k\}$ satisfy \eqref{stepsizes} with
$a=3/5$, and $b=2/5$.
Under Assumptions \ref{assump:HG_smooth_nonconvex}, we have for all $k\geq\Kcal$
\begin{align*}
    \min_{t\leq k}\mathbb{E}[\|\nabla f(\theta_t)\|^2] &\leq \frac{4}{\alpha_0(k+1)^{2/5}}\mathbb{E}[f(\theta_{\Kcal})-f^{\star}]+\frac{4L^2}{\beta_0\lambda_G (k+1)^{2/5}}\mathbb{E}[\|\omega_{\Kcal}-\omega^{\star}(\theta_{\Kcal})\|^2]\notag\\
    &\hspace{15pt}+\left(\frac{25L^2B^3\alpha_0^2}{2c_{\tau}}+\frac{2L^4 B^2 \alpha_0^3}{\lambda_G \beta_0^2}+\frac{L^2 \alpha_0\beta_0 C_2}{c_{\tau}\lambda_G}\right)\frac{8\tau_k^2\log(k+1)}{5\log(2)c_{\tau}(k+1)^{2/5}}.
\end{align*}
\end{thm}




\subsection{Technical Challenges \& Coupling between Decision and Auxiliary Variables}\label{subsec:tech_challenges}
The main technical challenge in analyzing Algorithm \ref{Alg:two-time-scale-SGD} is to handle the coupling between $\theta$, $\omega$,
% (two-time-scale updates) 
and the time-varying Markovian samples simultaneously. 
% It also worth noting that the Markovian samples affect the current update of $\theta$, which induces the Markov chain used to generate the future samples.
To illustrate the complications involved, we quickly look at how we might show $\|f(\theta_k)-f^{\star}\|^2\rightarrow 0$ in the case where $f$ observes the P\L~condition.
For the simplicity of notation, we define $z_k\triangleq\omega_k-\omega^{\star}(\theta_k)$ and
\begin{align}
\begin{aligned}
    &\widebar{\Delta H_{k}} \triangleq H(\theta_k,\omega_k,X_k)-H(\theta_k,\omega^{\star}(\theta_k),X_k)\\
    &\Delta H_k \triangleq H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\\
    &\Delta G_k \triangleq G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})].
    \end{aligned}
    \label{eq:Delta_z_def}
\end{align}
We can think of $\widebar{\Delta H_k}$ as the bias due to the inaccurate auxiliary variable and $\Delta H_{k}$ and $\Delta G_{k}$ as the errors that the Markovian samples cause to $H$ and $G$.


From the update rule \eqref{alg:update_theta} and the $L$-smoothness of the function $f$, we have 
\begin{align}
    &f(\theta_{k+1})\leq f(\theta_{k})+\langle\nabla f(\theta_k),\theta_{k+1}-\theta_k\rangle+\frac{L}{2}\|\theta_{k+1}-\theta_k\|^2\notag\\
    &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega_k,X_k)\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k,X_k)\|^2\notag\\
    % &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle\notag\\
    % &\hspace{20pt}-\alpha_k\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\notag\\
    &\hspace{20pt}-\alpha_k\left\langle\nabla f(\theta_k), \Delta H_k\hspace{-2pt}+\hspace{-2pt}\widebar{\Delta H_k}\right\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    &= f(\theta_{k})\hspace{-2pt}-\hspace{-2pt}\alpha_k\|\nabla f(\theta_k)\|^2\hspace{-2pt}-\hspace{-2pt}\alpha_k\left\langle\nabla f(\theta_k), \Delta H_k\hspace{-2pt}+\hspace{-2pt}\widebar{\Delta H_k}\right\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2,
    \label{prop:pl_nonconvex:eq1}
\end{align}
where the last equality follows from \eqref{operator:H}, i.e. $\nabla f(\theta_k)=\mathbb{E}_{\hat{X}\sim \mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]$. If the samples were i.i.d. and the auxiliary variables were always solved perfectly, we would have $\mathbb{E}[\Delta H_k]=\mathbb{E}[\widebar{\Delta H_k}]=0$, reducing the problem to the one studied in the standard SGD. The focus of our work is to investigate how the two terms can be properly controlled in the presence of the Markovian noise and inexact auxiliary variables. To analyze the term involving $\Delta H_k$ we leverage Assumptions \ref{assump:markov-chain} and \ref{assump:tv_bound}.
\begin{lem}
    For any $k\geq \tau_k$, we have
    \begin{align*}
    \mathbb{E}\left[-\left\langle\nabla f(\theta_k),\Delta H_k\right\rangle\right] &\leq 12L^2B^3\tau_k^2\alpha_{k-\tau_k}.
    \end{align*}
\label{lem:Gamma_bound}
\end{lem}
\begin{proof}
Our Markov process is a time-varying one (they depend on the iterates $\theta$). Therefore, one cannot directly utilize Assumption \ref{assump:markov-chain} to analyze the bias of $G$ in Algorithm \ref{Alg:two-time-scale-SGD} since the mixing time is defined for a fixed Markov chain (see Definition \ref{def:mixing_time}). To handle this difficulty, we introduce an auxiliary Markov chain $\{\widetilde{X}_{k}\}$ generated under the decision variable $\theta_{k-\tau_k}$ starting from $X_{k-\tau_{k}}$ as follows
\begin{align}
% X_{k-\tau_k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  
{X}_{k-\tau_k} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \widetilde{X}_{k-\tau_k+1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \cdots \widetilde{X}_{k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \widetilde{X}_{k}.
\label{eq:def_distribution_d}
\end{align}
% and we use $d_k$ to denote the distribution of $\widetilde{X}_{k}$. 
% Thus, one can apply Assumption \ref{assump:markov-chain} to $\{\widetilde{X}_{k}\}$. 
For clarity, we recall original the time-varying Markov processes $\{X_k\}$ generated by Algorithm~\ref{Alg:two-time-scale-SGD}
\begin{align*}
X_{k-\tau_k} \stackrel{\theta_{k-\tau_k+1}}{\longrightarrow} X_{k-\tau_k+1} \stackrel{\theta_{k-\tau_k+2}}{\longrightarrow} \cdots \stackrel{\theta_{k-1}}{\longrightarrow} X_{k-1} \stackrel{\theta_{k}}{\longrightarrow} X_{k}.
\end{align*}
Using the shorthand notation $y_k=\nabla f(\theta_k)$, we define the following quantities
\begin{align*}
    &T_1 = \mathbb{E}[\langle y_k-y_{k-\tau_k},\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]-H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle]\notag\\
    &T_2 = \mathbb{E}[\langle y_{k-\tau_k},H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)-H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle]\notag\\
    &T_3 = \mathbb{E}[\langle y_{k-\tau_k},H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\rangle]\notag\\
    &T_4 = \mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-2pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\bar{X})]-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\rangle]\notag\\
    &T_5 = \mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\hat{X})]\hspace{-2pt}-\hspace{-2pt}\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-4pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\bar{X})]\rangle]\notag\\
    &T_6 = \mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hat{X}]\rangle].
\end{align*}
It is easy to see that
\begin{align}
    -\mathbb{E}\left[\left\langle\nabla f(\theta_k),\Delta H_k\right\rangle\right]
    % &=-\mathbb{E}\big[\langle \nabla f(\theta_k),H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\big]\notag\\
    % &=-\mathbb{E}\big[\langle \nabla f(\theta_k)-\nabla f(\theta_{k-\tau_k}),H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\big]\notag\\
    % &\hspace{20pt}-\mathbb{E}\big[\langle \nabla f(\theta_{k-\tau_k}),H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\big]\notag\\
    &=T_1+T_2+T_3+T_4+T_5+T_6.
    \label{eq:bound_Gamma_breakdown}
\end{align}
We analyze the terms of \eqref{eq:bound_Gamma_breakdown} individually. First, we treat $T_1$ using the boundedness of $H$ and the Lipschitz continuity of $\nabla f$
\begin{align}
T_1&\leq \mathbb{E}\big[\left\|y_k-y_{k-\tau_k}\right\|\left\|H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\right\|\big]\notag\\
&\leq L\mathbb{E}\big[\left\|\theta_k-\theta_{k-\tau_k}\right\|\big]]\cdot 2B\leq2B^2 L\tau_k\alpha_{k-\tau_k},
\label{lem:Gamma_bound:T1}
\end{align}
where the last inequality follows from
\[\|\theta_k-\theta_{k-\tau_k}\|\leq\sum_{t=k-\tau_k}^{k}\|\alpha_t H(\theta_t,\omega_t,X_t)\|\leq B\tau_k\alpha_{k-\tau_k}.\]
% To bound $T_2$, we employ the boundedness $\nabla f$ and the Lipschitz continuity of $H$
Similarly, for $T_2$ we have
\begin{align}
    T_2&\leq \mathbb{E}\big[\|y_{k-\tau_k}\|\|H(\theta_k,\omega^{\star}(\theta_k),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\|\big]\notag\\
    &\leq B\mathbb{E}\big[\|H(\theta_k,\omega^{\star}(\theta_k),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\|\big]\notag\\
    &\leq BL\mathbb{E}\big[\|\theta_k-\theta_{k-\tau_k}\|+\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k-\tau_k})\|\big]\notag\\
    &\leq BL(L+1)\mathbb{E}\big[\|\theta_k-\theta_{k-\tau_k}\|\big]\leq B^2 L(L+1)\tau_k\alpha_{k-\tau_k}.
    \label{lem:Gamma_bound:T2}
\end{align}
To analyze $T_3$, we utilize the law of total expectation: given $\Fcal\subseteq\Fcal'$ and a random variable $X$ we have $\Eset[X\mid\Fcal] = \Eset[\Eset[X\mid\Fcal']\mid\Fcal]$.   

Let $\Fcal_k$ be $\Fcal_k=\{X_0,\ldots,X_k,\theta_0,\ldots,\theta_k,\omega_0,...,\omega_k\}$,
and for convenience we denote
\[p_{k}(x) = P(X_{k} = x\mid\Fcal_{k-1})\quad  \text{and}\quad  \tilde{p}_{k}(x) = P(\widetilde{X}_{k} = x\mid\Fcal_{k-1}).\]
Then, we have
\begin{align*}
    &\mathbb{E}\big[\left\langle y_{k-\tau_k},H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\right\rangle\mid \Fcal_{k-\tau_k}\big]\notag\\
    % &=\langle \nabla f(\theta_{k-\tau_k}),\mathbb{E}\big[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\mid \Fcal_{k-\tau_k}\big]\rangle\notag\\
    &\leq\left\| y_{k-\tau_k}\right\|\|\mathbb{E}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\mid \Fcal_{k-\tau_k}]\|\notag\\
    &=\left\|y_{k-\tau_k}\right\|\big\|\mathbb{E}\big[\mathbb{E}\big[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\hspace{-2pt}\mid\hspace{-2pt} \Fcal_{k-1}\big]\mid \Fcal_{k-\tau_k}\big]\big\|\notag\\
    &\leq B\mathbb{E}[\int_{\Xcal}H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),x)(p_k(x)-\widetilde{p}_k(x)) dx \mid \Fcal_{k-\tau_k}]\notag\\
    &\leq 2B^2 \mathbb{E}[d_{TV}(p_k(\cdot), \widetilde{p}_k(\cdot))\mid \Fcal_{k-\tau_k}]\notag\\
    &\leq 2B^2 \mathbb{E}\big[d_{TV}(p_{k-1}(\cdot),\widetilde{p}_{k-1}(\cdot))+L\|\theta_k-\theta_{k-\tau_k}\|\mid \Fcal_{k-\tau_k}\big],
\end{align*}
where the second inequality uses the definition of the TV distance in \eqref{eq:TV_def}, and the last inequality is a result of Assumption \ref{assump:tv_bound}. Recursively applying this inequality and taking the expectation, we get
\begin{align}
    T_3
    % &\leq 2B^2 \mathbb{E}\big[d_{TV}(p_{k-1}(\cdot),\widetilde{p}_{k-1}(\cdot))+L\|\theta_k-\theta_{k-\tau_k}\|\big]\notag\\
    &\leq 2B^2 L\sum_{t=k-\tau_k+1}^{k-1}\mathbb{E}[\|\theta_t-\theta_{k-\tau_k}\|]\leq 2B^3 L\tau_k^2\alpha_{k-\tau_k}.
    \label{lem:Gamma_bound:T3}
\end{align}
Similarly, to bound $T_4$, we again use the definition of TV distance
\begin{align*}
    &\mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\bar{X})]-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\rangle\mid\Fcal_{k-\tau_k}]\notag\\
    &\leq\left\|y_{k-\tau_k}\right\|\big\|\mathbb{E}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-2pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\bar{X})]\hspace{-2pt}\mid\hspace{-2pt}\Fcal_{k-\tau_k}]\big\|\notag\\
    &\leq B\cdot 2B \mathbb{E}[d_{TV}(\widetilde{p}_k(\cdot),\mu_{\theta_{k-\tau_k}})\mid \Fcal_{k-\tau_k}].
\end{align*}
Taking the expectation and using the definition of the mixing time \eqref{def:mixing_time},
\begin{align}
    T_4&\leq 2B^2 \mathbb{E}[d_{TV}(P(\widetilde{X}_k=\cdot),\mu_{\theta_{k-\tau_k}})]
    % \leq 2B^2 m\rho^{\tau_k}
    \leq 2B^2\alpha_k.
    \label{lem:Gamma_bound:T4}
\end{align}
We next consider $T_5$
\begin{align*}
    &\mathbb{E}[\langle y_{k-\tau_k},\hspace{-1pt}\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}\hspace{-1pt}(\theta_{k-\tau_k}),\hspace{-1pt}\hat{X})]\hspace{-2pt}-\hspace{-2pt}\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-6pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}\hspace{-1pt}(\theta_{k-\tau_k}),\hspace{-1pt}\bar{X})]\rangle\hspace{-2pt}\mid\hspace{-2pt}\Fcal_{k-\tau_k}]\notag\\
    &\leq B\|\mathbb{E}[\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-4pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\bar{X})]\hspace{-2pt}-\hspace{-2pt}\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\hat{X})]\hspace{-2pt}\mid\hspace{-2pt}\Fcal_{k-\tau_k}]\|\notag\\
    &\leq 2B^2\mathbb{E}[d_{TV}(\mu_{\theta_{k-\tau_k}},\mu_{\theta_k})\mid \Fcal_{k-\tau_k}],
\end{align*}
where the last inequality again comes from the definition of the TV distance in \eqref{eq:TV_def}. By \eqref{assump:tv_bound:eq2} in Assumption \ref{assump:tv_bound}, we have
\begin{align}
    T_5&\leq2B^2\mathbb{E}[d_{TV}(\mu_{\theta_{k-\tau_k}},\mu_{\theta_k})]\leq 2B^2 L\mathbb{E}[\|\theta_k-\theta_{k-\tau_k}\|]\leq 2B^3 L\tau_k\alpha_k.
    \label{lem:Gamma_bound:T5}
\end{align}
Finally, we bound $T_6$ using the boundedness of $\nabla f$ and the Lipschitz continuity of $H$
\begin{align*}
    &T_6\leq \mathbb{E}\big[\| y_{k-\tau_k}\|\|\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}\big[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hat{X})\big]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\big[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})\big]\big]\|\notag\\
    &\leq B L\mathbb{E}[\|\theta_{k-\tau_k}\hspace{-2pt}-\hspace{-2pt}\theta_k\|\hspace{-2pt}+\hspace{-2pt}\|\omega^{\star}(\theta_{k-\tau_k})\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_k)\|]\leq 2L^2B \mathbb{E}[\|\theta_{k-\tau_k}\hspace{-2pt}-\hspace{-2pt}\theta_k\|]\leq 2L^2B^2\tau_k\alpha_{k-\tau_k}.
    % \label{lem:Gamma_bound:T6}
\end{align*}
The claimed result follows from plugging the bounds on $T_1$-$T_6$ into \eqref{eq:bound_Gamma_breakdown}.
\end{proof}



In addition, we can use the Lipschitz continuity of $H$ to study the error caused by $\widebar{\Delta H_k}$ and show that it can be bounded by the sum of $\|\theta_k-\theta^{\star}\|^2$ and $\|z_k\|^2$. This bound on $\widebar{\Delta H_k}$ together with the bound on $\Delta H_k$ established in Lemma~\ref{lem:Gamma_bound} leads to the following proposition on the step-wise convergence of $\mathbb{E}[f(\theta_{k})-f^{\star}]$.
\begin{prop}\label{prop:pl_nonconvex}
Under Assumptions \ref{assump:HG_smooth}-\ref{assump:tv_bound}, we have for all $k\geq\Kcal$
\begin{align*}
    \mathbb{E}[f(\theta_{k+1})-f^{\star}]\leq (1\hspace{-2pt}-\hspace{-2pt}\lambda_f\alpha_k)\mathbb{E}[f(\theta_{k})-f^{\star}]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k}.
\end{align*}
\end{prop}
\begin{proof}
% We introduce the following technical lemma that bounds the a cross-term related to $\Delta H_k$. We skip the proof of Lemma~\ref{lem:Gamma_bound} due to its similarity to a lemma that we will later introduce and prove.

By the Lipschitz condition of the operator $H$,
\begin{align*}
    -\mathbb{E}[\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle] &\leq\frac{1}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2+\|H(\theta_k, \omega_k, X_k)-H(\theta_k, \omega^{\star}(\theta_k), X_k)\|^2]\notag\\
    &\leq\frac{1}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2}{2}\mathbb{E}\left[\|z_k\|^2\right].
\end{align*}
% \begin{align*}
%     \left\|\widebar{\Delta H_k}\right\|&=\left\|H(\theta_k, \omega_k, X_k)-H(\theta_k, \omega^{\star}(\theta_k), X_k)\right\|\leq L\left\|z_k\right\|,
% \end{align*}
% which implies
% \begin{align*}
%     -\mathbb{E}[\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle] &\leq\frac{1}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2}{2}\mathbb{E}\left[\|z_k\|^2\right].
% \end{align*}
Using this inequality along with Lemma \ref{lem:Gamma_bound} in \eqref{prop:pl_nonconvex:eq1}, we have for all $k\geq \tau_k$ 
\begin{align*}
    \mathbb{E}[f(\theta_{k+1})]&\leq \mathbb{E}[f(\theta_{k})]-\alpha_k\left\langle\nabla f(\theta_k), \Delta H_k\right\rangle-\alpha_k\mathbb{E}[\|\nabla f(\theta_k)\|^2]\notag\\
    &\hspace{20pt}-\alpha_k\mathbb{E}\left[\left\langle\nabla f(\theta_k), \widebar{\Delta H_k}\right\rangle\right]+\frac{L B^2\alpha_k^2}{2}\notag\\
    &\leq \mathbb{E}[f(\theta_{k})]+12L^2B^3\tau_k^2\alpha_k\alpha_{k-\tau_k}-\alpha_k\mathbb{E}[\|\nabla f(\theta_k)\|^2]\notag\\
    &\hspace{20pt}+ \frac{\alpha_k}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{L B^2 \alpha_k^2}{2}\notag\\
    &\leq \mathbb{E}[f(\theta_{k})]-\frac{\alpha_k}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k}\notag\\
    &\leq \mathbb{E}[f(\theta_{k})]-\lambda_f\alpha_k\mathbb{E}\left[f(\theta_k)-f^{\star}\right]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k},
\end{align*}
where the last inequality is due to the P\L~condition.
Subtracting $f^{\star}$ from both sides of the inequality leads to the claimed result.
\end{proof}


Proposition~\ref{prop:pl_nonconvex} shows how the convergence of the decision variable depends on the precision of the auxiliary variable. We next aim to study how auxiliary variable evolves. Due to the assumption that the operator $H$ is bounded, the difference between $\theta_k$ and $\theta_{k-\tau_k}$ can be easily controlled by $\alpha_{k-\tau_k}$. However, the operator $G$ may not be bounded, and to properly handle $\|\omega_k-\omega_{k-\tau_k}\|$ we introduce the following lemma.
\begin{lem}\label{lem:omega_k-omega_k-tau}
For all $k\geq\tau_k$, we have 
\begin{align*}
\|\omega_k-\omega_{k-\tau_k}\|&\leq 3D\beta_{k-\tau_k}\tau_k\left(\|\omega_{k}\| +\|\theta_{k}\|+1\right).
% \notag\\
% &\leq \frac{1}{2}\left(\|\omega_{k}\| +\|\theta_{k}\|+1\right),
\end{align*}
% and
% \begin{align*}
%     \|\omega_k-\omega_{k-\tau_k}\|^2\leq \frac{3}{4}\left(\|\omega_{k}\|^2 +\|\theta_{k}\|^2+1\right).
% \end{align*}
\end{lem}
\begin{proof}
As a result of \eqref{eq:G_affinelybounded_D}, for any $k\geq 0$
\begin{align}
    \|\omega_{k+1}\|\hspace{-2pt}-\hspace{-2pt}\|\omega_{k}\|&\leq \|\omega_{k+1}\hspace{-2pt}-\hspace{-2pt}\omega_{k}\|\hspace{-2pt}=\hspace{-2pt}\|\beta_k G(\theta_{k+1},\omega_k,X_k)\|\hspace{-2pt}\leq\hspace{-2pt} D\beta_k\left(\|\theta_{k+1}\|\hspace{-2pt}+\hspace{-2pt}\|\omega_k\|\hspace{-2pt}+\hspace{-2pt}1\right).
    \label{lem:omega_k-omega_k-tau:ineq0}
\end{align}
% which leads to
% \begin{align*}
%     \|\omega_{k+1}\|&\leq(1+D\beta_k)\|\omega^{k}\|+D\beta_k (\|\theta_{k+1}\|+1).
% \end{align*}
Define $h_k=\|\omega_{k}\|+\|\theta_{k+1}\|$. We have for all $k\geq 1$
\begin{align*}
    h_k&=\|\omega_{k-1}+\beta_{k-1}G(\theta_k,\omega_{k-1},X_{k-1})\|+\|\theta_k+\alpha_k H(\theta_k,\omega_k,X_k)\|\notag\\
    &\leq \|\omega_{k-1}\|+D\beta_{k-1}(\|\theta_{k}\|+\|\omega_{k-1}\|+1)+\|\theta_k\|+B\alpha_k\notag\\
    &\leq (1+D\beta_{k-1})h_{k-1}+(B+D)\beta_{k-1}
\end{align*}
where the second inequality follows from \eqref{eq:G_affinelybounded_D} and Assumption \ref{assump:HG_smooth}, and the last inequality is due to $\alpha_k\leq\beta_k$ and the fact that $\{\beta_k\}$ is a decaying sequence.

Since $1+x \leq e^{x}$ for all $x\geq 0$, we have for all $k\geq\tau_k$ and $k-\tau_k\leq t\leq k$
\begin{align*}
    h_t&\leq (1+D\beta_{t-1})h_{t-1}+(B+D)\beta_{t-1}\notag\\
    &\leq (1+D\beta_{k-\tau_k})^{\tau_k+t-k} h_{k-\tau_k}+(B+D)\beta_{k-\tau_k}\sum_{t'=k-\tau_k}^{t-1}(1+D\beta_{k-\tau_k})^{t-t'-1}\notag\\
    &\leq (1+D\beta_{k-\tau_k})^{\tau_k} h_{k-\tau_k}+(B+D)\beta_{k-\tau_k}\tau_k(1+D\beta_{k-\tau_k})^{\tau_k}\notag\\
    &\leq e^{D\beta_{k-\tau_k}\tau_k}h_{k-\tau_k}+(B+D)\beta_{k-\tau_k}\tau_k e^{D\beta_{k-\tau_k}\tau_k}\leq 2h_{k-\tau_k}+\frac{1}{3},
\end{align*}
where the last inequality follows from the step size $2(B+D)\beta_{k-\tau_k}\tau_k\leq\frac{1}{3}\leq\log(2)$.
% 
Combining this inequality with \eqref{lem:omega_k-omega_k-tau:ineq0}, we have for all $k\geq\tau_k$
\begin{align*}
    &\|\omega_k-\omega_{k-\tau_k}\|\leq \sum_{t=k-\tau_k}^{k-1}\hspace{-3pt}\|\omega_{t+1}-\omega_t\| \leq D\hspace{-3pt}\sum_{t=k-\tau_k}^{k-1}\hspace{-3pt}\beta_{t}\left(h_t + 1\right) \leq D\beta_{k-\tau_k}\hspace{-3pt}\sum_{t=k-\tau_k}^{k-1}\hspace{-3pt}\big(2h_{k-\tau_k} + \frac{4}{3}\big) \notag\\
    &\leq\hspace{-2pt} 2D\beta_{k-\tau_k}\hspace{-2pt}\tau_k(\|\omega_{k-\tau_k}\| \hspace{-2pt}+\hspace{-2pt}\|\theta_{k-\tau_k+1}\|\hspace{-2.5pt}+\hspace{-2.5pt} \frac{2}{3}) \hspace{-2pt}\leq\hspace{-2pt} 2D\beta_{k-\tau_k}\hspace{-2pt}\tau_k(\|\omega_{k-\tau_k}\| \hspace{-2pt}+\hspace{-2pt}\|\theta_{k}\|\hspace{-2pt}+\hspace{-2pt}B\beta_{k-\tau_k}\hspace{-2pt}(\tau_k\hspace{-2pt}-\hspace{-2pt}1)\hspace{-2.5pt}+\hspace{-2.5pt} \frac{2}{3})\notag\\
    &\leq 2D\beta_{k-\tau_k}\tau_k\left(\|\omega_k-\omega_{k-\tau_k}\|+\|\omega_{k}\| +\|\theta_{k}\|+1\right).
\end{align*}
% where in the last inequality we use $2B\beta_{k-\tau_k}\tau_k\leq \frac{1}{3}$ again.
Re-arranging terms and again using the step size condition $2D\beta_{k-\tau_k}\tau_k\leq\frac{1}{3}$, we get
\begin{align*}
\|\omega_k-\omega_{k-\tau_k}\|&\leq 3D\beta_{k-\tau_k}\tau_k\left(\|\omega_{k}\| +\|\theta_{k}\|+1\right).
\end{align*}
\end{proof}

We now present Proposition~\ref{prop:auxiliary}, which reveals the effect of the decision variables on the convergence of the auxiliary variable.
\begin{prop}\label{prop:auxiliary}
% Let the step size sequence $\{\beta_k\}$ satisfy the condition for all $k\geq \tau_{k}$
% \begin{align}
%     \tau_k^2\beta_{k-\tau_k}\leq\min\left\{1,\frac{1}{6LB},\frac{\lambda_G}{22C_1+32D^2}\right\}.
%     \label{eq:stepsize_auxiliary}
% \end{align}
Under Assumptions \ref{assump:HG_smooth}-\ref{assump:tv_bound}, we have for all $k\geq\Kcal$
\begin{align*}
    \mathbb{E}[\|z_{k+1}\|^2] &\leq (1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_G\beta_k}{2})\mathbb{E}[\|z_{k}\|^2]\hspace{-2pt}+\hspace{-2pt}C_2\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}+C_2\tau_k^2\beta_{k-\tau_k}\beta_k.
\end{align*}
\end{prop}
\begin{proof}

We introduce a technical lemma that bounds the error in the auxiliary variable caused by the Markovian samples. We skip the proof of this lemma due to its similarity to that of Lemma~\ref{lem:Gamma_bound} and refer interested readers to the companion paper \cite{zeng2021two} for the full proof details.
\begin{lem}\label{lem:Lambda_bound}
    Recall the definition of $C_1$ in \eqref{notation:constant_C}. For any $k\geq\tau_k$, we have
    \begin{align*}
    \mathbb{E}[\langle z_k, \Delta G_k\rangle]\leq C_1\tau_k^2\beta_{k-\tau_k}\mathbb{E}\left[\|z_{k-\tau_k}\|^2+\|\theta_k\|^2+\|\omega_k\|^2+1\right].
\end{align*}
\end{lem}

Recall that $z_{k} = \omega_{k} - \omega^{\star}(\theta_{k})$. Using \eqref{alg:update_omega}, we have
\begin{align*}
    \|z_{k+1}\|^2
    % &=\|\omega_{k+1}-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    &= \|\omega_k+\beta_k G(\theta_{k+1},\omega_k, X_k)-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    &= \|\left(\omega_k-\omega^{\star}(\theta_k)\right)+\beta_k G(\theta_{k+1},\omega_k,X_k)+\left(\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\right)\|^2\notag\\
    % &= \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)\rangle+2\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle\notag\\
    % &\qquad + \|\beta_kG(\theta_{k+1},\omega_k,X_k)+ \omega^{\star}(\theta^k)-\omega^{\star}(\theta^{k+1})\|^2\notag\\
    &\leq \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)\rangle+2\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle\notag\\
    &\qquad + 2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2+2\|\omega^{\star}(\theta^k)-\omega^{\star}(\theta^{k+1})\|^2.
\end{align*}

% Recall from \eqref{eq:Delta_z_def} that $\Delta G_k = G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]$. Using this in the equation above,
From the definition of $\Delta G_k$ in \eqref{eq:Delta_z_def},
\begin{align}
    \|z_{k+1}\|^2&\leq \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle+2\beta_k\langle z_k,G(\theta_{k},\omega_k,X_k)\rangle\notag\\
    &\quad+2\langle z_k,\omega^{\star}(\theta_k)\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k+1})\rangle\hspace{-2pt} + \hspace{-2pt}2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2\hspace{-2pt}+\hspace{-2pt}2\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    % &= \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle \rangle\notag\\
    % &\quad+ 2\beta_k\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle+2\beta_k\langle z_k,\Delta G_{k}\rangle \hspace{-2pt}+\hspace{-2pt} 2\langle z_k,\omega^{\star}(\theta_k)\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k+1})\rangle  \notag\\ 
    % &\quad + 2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2 + 2\|\omega^{\star}(\theta^k)-\omega^{\star}(\theta^{k+1})\|^2\notag\\
    &\leq \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle\rangle\notag\\
    &\quad + 2\beta_k\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle \hspace{-2pt}+\hspace{-2pt} 2\beta_k\langle z_k,\Delta G_{k}\rangle + 2\langle z_k,\omega^{\star}(\theta_k)\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k+1})\rangle \notag\\
    &\quad+2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2+2L^2 B^2\alpha_k^2,
    \label{prop:auxiliary_eq1}
\end{align}
where the second inequality applies Assumption \ref{assump:HG_smooth} and \eqref{alg:update_theta}, i.e.,
\begin{equation}
 \|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\|^2 \leq  L^2 \|\theta_k-\theta_{k+1}\|^2= L^2\|\alpha_k H(\theta_k,\omega_k,X_k)\|^2 \leq L^2B^2\alpha_k^2.
    \label{prop:auxiliary_eq1.5}
\end{equation}
We next analyze each term on the right-hand side of \eqref{prop:auxiliary_eq1}. First, using the relation $\langle 2v_1,v_2\rangle\leq c\|v_1\|^2+\frac{1}{c}\|v_2\|^2$ for any vectors $v_1,v_2$ and scalar $c>0$, we bound the second term of \eqref{prop:auxiliary_eq1}
\begin{align}
    &\langle z_k,\hspace{-1pt}G(\theta_{k+1},\omega_k,\hspace{-1pt}X_k)\hspace{-2pt}-\hspace{-2pt}G(\theta_{k},\omega_k,\hspace{-1pt}X_k)\rangle\hspace{-2pt}\leq\hspace{-2pt} \frac{\lambda_G}{4}\|z_k\|^2\hspace{-2pt}+\hspace{-2pt}\frac{1}{\lambda_G}\|G(\theta_{k+1},\omega_k,\hspace{-1.5pt}X_k)\hspace{-2pt}-\hspace{-2pt}G(\theta_{k},\omega_k,\hspace{-1.5pt}X_k)\|^2\notag\\
    &\leq \frac{\lambda_G}{4}\|z_k\|^2+\frac{L^2}{\lambda_G}\|\theta_{k+1}-\theta_{k}\|^2 \leq \frac{\lambda_G}{4}\|z_k\|^2+\frac{L^2 B^2\alpha_k^2}{\lambda_G},\label{prop:auxiliary_eq1a}
\end{align}
where the second inequality follows from the Lipschitz continuity of $G$ and the last inequality is due to \eqref{prop:auxiliary_eq1.5}. Similarly, we consider the fifth term of \eqref{prop:auxiliary_eq1}
\begin{align}
    &2\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle\leq \frac{\beta_k\lambda_G}{2}\|z_k\|^2+\frac{2}{\lambda_G\beta_k}\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    &\leq \frac{\beta_k\lambda_G}{2}\|z_k\|^2+\frac{2L^2}{\lambda_G\beta_k}\|\theta_k-\theta_{k+1}\|^2\leq \frac{\beta_k\lambda_G}{2}\|z_k\|^2+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}.\label{prop:auxiliary_eq1b}
\end{align}
Next, using Assumption \ref{assump:stronglymonotone_G} and $z_{k} = \omega_{k} - \omega^{\star}(\theta_{k})$ we consider the third term of \eqref{prop:auxiliary_eq1}
\begin{align}
    2\beta_k\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle \leq -2\lambda_G\beta_k\|z_k\|^2.\label{prop:auxiliary_eq1c}
\end{align}
By \eqref{eq:G_affinelybounded_D}  and \eqref{alg:update_theta} we have
\begin{align}
\|G(\theta_{k+1},\omega_{k},X_{k})\|^2 \hspace{-2pt}\leq \hspace{-2pt}2D^2 \big(\|\theta_{k+1}\| \hspace{-2pt}+\hspace{-2pt} \|\omega_{k}\| + 1\big)^2\hspace{-2pt}\leq \hspace{-2pt}  2D^2 \big(\|\theta_{k}\| \hspace{-2pt}+\hspace{-2pt} B\alpha_{k} + \|\omega_{k}\| \hspace{-2pt}+\hspace{-2pt} 1\big)^2.\label{prop:auxiliary_eq1d}
% &\quad\leq 2D^2\beta_{k}^2 \big(\|\theta_{k}\| + B\alpha_{k} + \|\omega_{k}-\omega^{\star}(\theta_{k})\| + \|\omega^{\star}(\theta_{k})\| + 1\big)^2\notag\\
% &\quad \leq 2D^2\beta_{k}^2 \big((1+D)\|\theta_{k}\| + B\alpha_{k} + \|z_{k}\| + D + 1\big)^2,
\end{align}
Taking the expectation on both sides of \eqref{prop:auxiliary_eq1} and using \eqref{prop:auxiliary_eq1a}--\eqref{prop:auxiliary_eq1d} and Lemma \ref{lem:Lambda_bound}
\begin{align}
    \mathbb{E}[\|z_{k+1}\|^2]
    % &\leq \mathbb{E}[\|z_k\|^2]+2\beta_k\mathbb{E}[\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle]\notag\\
    % &\quad+2\beta_k\mathbb{E}[\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle]+2\beta_k\mathbb{E}[\left\langle z_k, \Delta G_k\right\rangle]\notag\\
    % &\quad+2\mathbb{E}[\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle]+6D^2\beta_k^2(\|\theta_{k+1}\|^2+\|\omega_k\|^2+1)+2L^2 B^2 \alpha_k^2\notag\\
    &\leq \mathbb{E}[\|z_k\|^2]+\frac{\beta_k\lambda_G}{2}\mathbb{E}[\|z_k\|^2]+\frac{2L^2 B^2 \beta_k\alpha_k^2}{\lambda_G}+\frac{\beta_k\lambda_G}{2}\mathbb{E}[\|z_k\|^2]+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}\notag\\
    &\quad-2\lambda_G\beta_k\mathbb{E}[\|z_k\|^2]+C_1\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k-\tau_k}\|^2+\|\theta_k\|^2+\|\omega_k\|^2+1\right]\notag\\
    &\quad + 2D^2\beta_{k}^2 \big(\|\theta_{k}\| + B\alpha_{k} + \|\omega_{k}\| + 1\big)^2 + 2L^2 B^2\alpha_k^2\notag\\
    &\leq (1-\lambda_G\beta_k)\mathbb{E}[\|z_k\|^2]+C_1\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k-\tau_k}\|^2\right]\notag\\
    &\quad+(C_1+8D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2+\|\omega_k\|^2\right]\notag\\
    &\quad+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}+(C_1+32D^2+\frac{2L^2 B^2}{\lambda_G}+2L^2 B^2)\tau_k^2\beta_{k-\tau_k}\beta_k,
    \label{prop:auxiliary_eq2}
\end{align}
where the last inequality uses $\alpha_k\leq\beta_k$ and $B\alpha_k\leq 1$.  Note that $\|z_{k-\tau_k}\|^2$ obeys
\begin{align*}
    \|z_{k-\tau_k}\|^2&=\|z_k-(\omega_k-\omega_{k-\tau_k})+(\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k-\tau_k}))\|^2\notag\\
    &\leq 3\left(\|z_k\|^2+\|\omega_k-\omega_{k-\tau_k}\|^2+\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k-\tau_k})\|^2\right)\notag\\
    &\leq 3\|z_k\|^2+\frac{9}{4}\left(\left\|\omega_{k}\right\|^{2}+\left\|\theta_{k}\right\|^{2}+1\right)+L^2\|\theta_{k}-\theta_{k-\tau_k}\|^2\notag\\
    &\leq 3\left(\|z_k\|^2+\|\omega_{k}\|^{2}+\|\theta_{k}\|^{2}\right)+L^2 B^2\tau_k^2\alpha_{k-\tau_k}^2+\frac{9}{4}\notag\\
    &\leq 3\left(\|z_k\|^2+\|\omega_{k}\|^{2}+\|\theta_{k}\|^{2}+1\right),
\end{align*}
where the second inequality is due to Lemma \ref{lem:omega_k-omega_k-tau} and the Lipschitz continuity of $\omega^{\star}$, and the last inequality follows from the step size condition $L B\tau_k\alpha_{k-\tau_k}\leq\frac{1}{6}$. Substituting the preceding relation into \eqref{prop:auxiliary_eq2}, we have for all $k\geq\tau_k$
\begin{align}
    \mathbb{E}[\|z_{k+1}\|^2] &\leq (1-\lambda_G\beta_k)\mathbb{E}[\|z_k\|^2]+3C_1\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k}\|^2\right]\notag\\
    &\quad+(4C_1+8D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2+\|\omega_k\|^2\right]\notag\\
    &\quad+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}+(4C_1+32D^2+\frac{2L^2 B^2}{\lambda_G}+2L^2 B^2)\tau_k^2\beta_{k-\tau_k}\beta_k\notag\\
    &\leq (1-\lambda_G\beta_k)\mathbb{E}[\|z_k\|^2]+(11C_1+16D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k}\|^2\right]\notag\\
    &\quad+(4D^2+1)(4C_1+8D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2\right]+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}\notag\\
    &\quad+((4D^2+1)(4C_1+32D^2)+\frac{2L^2 B^2}{\lambda_G}+2L^2 B^2)\tau_k^2\beta_{k-\tau_k}\beta_k,
    \label{prop:auxiliary_eq2.5}
\end{align}
where in the last inequality we use \eqref{eq:G_affinelybounded_D} to derive 
\begin{align*}
    \|\omega_k\|^2\hspace{-2pt}\leq \hspace{-2pt}2\|\omega_{k}\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k})\|^2\hspace{-2pt}+\hspace{-2pt}2\|\omega^{\star}(\theta_{k})\|^2\hspace{-2pt}\leq\hspace{-2pt} 2\|z_k\|^2\hspace{-2pt}+\hspace{-2pt}2D^2(\|\theta_k\|\hspace{-2pt}+\hspace{-2pt}1)^2\hspace{-2pt}\leq\hspace{-2pt} 2\|z_k\|^2\hspace{-2pt}+\hspace{-2pt}4D^2(\|\theta_k\|^2\hspace{-2pt}+\hspace{-2pt}1).
\end{align*}
By the choice of the step size we have $(11C_1+16D^2)\tau_k^2\beta_{k-\tau_k}\leq\frac{\lambda_G}{2}$. Thus, using the constant $C_2$ defined in \eqref{notation:constant_C}, \eqref{prop:auxiliary_eq2.5} implies
\begin{align*}
    \mathbb{E}[\|z_{k+1}\|^2] \leq(1-\frac{\lambda_G\beta_k}{2})\mathbb{E}[\|z_k\|^2]+C_2\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2+1\right]+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}.
\end{align*}
\end{proof}

As mentioned earlier, the update of the auxiliary variable occurs at a faster time scale, i.e.\ $\alpha_{k} \ll \beta_{k}$, in order to provide a more accurate gradient for the update of $\theta_k$.
Propositions~\ref{prop:pl_nonconvex} and \ref{prop:auxiliary} show that the convergence of the decision variable and the auxiliary variable forms a coupled dynamical system that evolves under two different rates. To characterize the  coupling of the two iterates and analyze the finite-time complexity, we consider the following Lyapunov function 
\begin{equation*}
    V(\theta_{k},\omega_{k}) = \Eset[f(\theta_{k})-f^{\star}] + (\alpha_{k}/\beta_{k})\Eset[\|\omega_{k}-\omega^{\star}(\theta_{k})\|^2].    
\end{equation*}
We will derive the finite-time convergence rate of $V(\theta_k,\omega_k)$ to 0, which immediately translates to the convergence rates for $\Eset[f(\theta_{k})-f^{\star}]$ and $\Eset[\|\omega_{k}-\omega^{\star}(\theta_{k})\|^2]$.





\subsection{Two-Time-Scale Lemma}
\label{sec:lyapunov_lemma}
Although we analyze the performance of our algorithm for different types of objective functions and with different convergence metrics, these analyses eventually reduce to the study of two coupled inequalities. The dynamics of these two inequalities happen on different time scales determined by the two step sizes used in our algorithm. 
%
In this section we present a general result, which we call the two-time-scale lemma, that characterizes the behavior of these coupled inequalities. \looseness=-1
% This lemma gives us a tool for a unified analysis for different types of objectives $f$, and may be of further interest to the study of the finite-time performance of multiple-time-scale dynamical systems apart from those considered in this paper. 






\begin{lem}\label{lem:lyapunov}
    Let $\{a_k,\, b_k,\,c_k,\,d_k,\,e_k,\,f_k\}$ be non-negative 
    % and constant 
    sequences satisfying $\frac{a_{k+1}}{d_{k+1}}\leq\frac{a_{k}}{d_{k}} < 1$, for all $k\geq0$.
    Let $\{x_k\}, \{y_k\}$ be two non-negative sequences. We consider two settings on their dynamics. 
\begin{enumerate}[leftmargin = 4.5mm]
    \item  Suppose that $x_{k},y_{k}$ satisfy the following coupled inequalities
    \begin{align}
    x_{k+1}\leq(1-a_k)x_k+b_k y_k+c_k,\quad y_{k+1}\leq(1-d_k)y_k+e_k x_k+f_k.\label{lem:lyapunov:sc:def}
    \end{align}
    In addition, assume that there exists a constant $A\in\mathbb{R}$ such that  
    \begin{align}
    Aa_k-b_k-\frac{A a_k^2}{d_k}\geq 0\quad \text{and}\quad  \frac{A e_k}{d_{k}}\leq\frac{1}{2}, \quad \text{for all } k\geq0. \label{lem:lyapunov:sc:def3}
    \end{align}
    Then we have  for all $0 \leq \tau \leq k$
    \begin{align*}
    x_k&\leq (x_{\tau}+\frac{A a_{\tau} }{d_{\tau}}y_{\tau})\prod_{t=\tau}^{k-1}(1-\frac{a_t}{2})+\sum_{\ell=\tau}^{k-1}\Big(c_{\ell}+\frac{A a_{\ell} f_{\ell}}{d_{\ell}}\Big) \prod_{t=\ell+1}^{k-1}(1-\frac{a_t}{2}).
    \end{align*}
    
    \item  Suppose that $\{x_k,y_k\}$ satisfy the following coupled inequalities
    \begin{align}
    x_{k+1}\leq(1+a_k)x_k+b_k y_k+c_k,\quad y_{k+1}\leq(1-d_k)y_k+e_k x_k+f_k.\label{lem:lyapunov:def}
    \end{align}    
    $\{u_k\}$ is a non-negative sequence such that
    \begin{align}
        u_k\leq(1+a_k)x_k-x_{k+1}+b_k y_k+c_k,\label{lem:lyapunov:def3}
    \end{align}
    then we have for any $0 \leq \tau \leq k$
    \begin{align*}
    \sum_{t=\tau}^{k}u_t \leq \Big(1+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})e^{\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})}\Big)\Big(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\Big).
\end{align*}
\end{enumerate}    
\end{lem}
\begin{proof}
Case 1) Consider $V_k=x_k+\frac{A a_k}{d_k}y_k$. From the second equation in \eqref{lem:lyapunov:sc:def},
\begin{align*}
    \frac{A a_{k+1}}{d_{k+1}}y_{k+1} &\leq \frac{A a_{k}}{d_{k}}y_{k+1} \leq \frac{A a_{k}}{d_{k}}\left((1-d_k)y_k+e_k x_k+f_k\right)\notag\\
    &= (1-a_k)\frac{A a_{k}}{d_{k}}y_k+(a_k-d_k)\frac{A a_{k}}{d_{k}}y_k+\frac{A a_{k}e_k x_k}{d_{k}}+\frac{A a_{k} f_k}{d_{k}}.
\end{align*}
Combining this with the first inequality of \eqref{lem:lyapunov:sc:def} yields
\begin{align*}
    V_{k+1}&=x_{k+1}+\frac{A a_{k+1}}{d_{k+1}}y_{k+1}\notag\\
    &\leq (1\hspace{-2pt}-\hspace{-2pt}a_k)x_k\hspace{-2pt}+\hspace{-2pt}b_k y_k\hspace{-2pt}+\hspace{-2pt}c_k\hspace{-2pt}+\hspace{-2pt}(1\hspace{-2pt}-\hspace{-2pt}a_k)\frac{A a_{k}}{d_{k}}y_k\hspace{-2pt}+\hspace{-2pt}(a_k\hspace{-2pt}-\hspace{-2pt}d_k)\frac{A a_{k}}{d_{k}}y_k\hspace{-2pt}+\hspace{-2pt}\frac{A a_{k}e_k x_k}{d_{k}}\hspace{-2pt}+\hspace{-2pt}\frac{A a_{k} f_k}{d_{k}}\notag\\
    &= (1-a_k)\left(x_k+\frac{A a_k y_k}{d_k}\right)+\left(\frac{A a_k^2}{d_k}-A a_k+b_k\right)y_k+c_k+\frac{A a_{k}e_k x_k}{d_{k}}+\frac{A a_{k} f_k}{d_{k}}\notag\\
    &\leq (1-a_k)V_k+\frac{a_k}{2}x_k+c_k+\frac{A a_{k} f_k}{d_{k}}\leq (1-\frac{a_k}{2})V_k+c_k+\frac{A a_{k} f_k}{d_{k}},
\end{align*}
where the second inequality follows from \eqref{lem:lyapunov:sc:def3}.
Applying this relation recursively,
\begin{align*}
    x_k&\leq V_k\leq V_{\tau}\prod_{t=\tau}^{k-1}(1-\frac{a_t}{2})+\sum_{\ell=\tau}^{k-1}\left(c_{\ell}+\frac{A a_{\ell} f_{\ell}}{d_{\ell}}\right) \prod_{t=\ell+1}^{k-1}(1-\frac{a_t}{2})\\
    &\leq (x_{\tau}+\frac{A a_{\tau} }{d_{\tau}}y_{\tau})\prod_{t=\tau}^{k-1}(1-\frac{a_t}{2})+\sum_{\ell=\tau}^{k-1}\left(c_{\ell}+\frac{A a_{\ell} f_{\ell}}{d_{\ell}}\right) \prod_{t=\ell+1}^{k-1}(1-\frac{a_t}{2}).
\end{align*}


Case 2) Re-arranging the second inequality of \eqref{lem:lyapunov:def} and multiplying by $\frac{b_k}{d_k}$, we get\looseness=-1
\begin{align*}
    b_k y_k\leq \frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+\frac{b_k e_k x_k}{d_k}+\frac{b_k f_k}{d_k}.
\end{align*}
Plugging this inequality into the first inequality of \eqref{lem:lyapunov:def} yields
\begin{align}
    x_{k+1}&\leq(1+a_k)x_k+c_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+\frac{b_k e_k x_k}{d_k}+\frac{b_k f_k}{d_k}\notag\\
    &\leq(1+g_k)x_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+c_k+\frac{b_k f_k}{d_k},
    \label{lem:lyapunov:eq3}
\end{align}
where we define $g_k=a_k+\frac{b_k e_k}{d_k}$.
Since $1+c\leq\exp(c)$ for any scalar $c>0$, we have
\begin{align}
    x_{k+1}
    % &\leq(1+a_k+\frac{b_k e_k}{d_k})x_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+c_k+\frac{b_k f_k}{d_k}\notag\\
    &\leq\exp(g_k)x_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+c_k+\frac{b_k f_k}{d_k}\notag\\
    &\leq\exp(\sum_{t=\tau}^{k}g_t)x_{\tau}+\exp\big(\sum_{t=\tau}^{k}g_t\big)\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
    &\leq \exp(\sum_{t=\tau}^{k}g_t)\Big(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\Big),
    \label{lem:lyapunov:eq4}
\end{align}
where the second inequality applies the first inequality recursively. 
% This bound implies
% \begin{align}
%     \max_{\tau\leq t\leq k}x_t &\leq \exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))x_{\tau}\notag\\
%     &\hspace{20pt}+\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
%     &\leq \exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right).
%     \label{lem:lyapunov:eq4}
% \end{align}
The inequalities \eqref{lem:lyapunov:eq3}, \eqref{lem:lyapunov:eq4}, and \eqref{lem:lyapunov:def3} together imply
\begin{align*}
    \sum_{t=\tau}^{k}u_t&\leq \sum_{t=\tau}^{k}(x_t-x_{t+1})+\big(\hspace{-2pt}\max_{\tau\leq t\leq k}x_t\big)\hspace{-2pt}\sum_{t=\tau}^{k}g_t+\hspace{-2pt}\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
    &\leq x_{\tau}\hspace{-1pt}+\hspace{-2pt}\sum_{t=\tau}^{k}g_t\exp\big(\sum_{t=\tau}^{k}g_t\big)\Big(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\Big)+\frac{b_{\tau}}{d_{\tau}}y_{\tau}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\notag\\
    &=\left(1+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\right)\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right).
\end{align*}
% \begin{align*}
%     \sum_{t=\tau}^{k}u_t &\leq \sum_{t=\tau}^{k}(x_t-x_{t+1})+\big(\hspace{-2pt}\max_{\tau\leq t\leq k}x_t\big)\hspace{-2pt}\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))+\hspace{-2pt}\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
%     &\leq x_{\tau}+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right)\notag\\
%     &\hspace{20pt}+\frac{b_{\tau}}{d_{\tau}}y_{\tau}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\notag\\
%     &=\left(1+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\right)\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right).
% \end{align*}
\end{proof}

Lemma \ref{lem:lyapunov} studies the behavior of the two interacting sequences $\{x_k\}$ and $\{y_k\}$ that have generic structure. In our analysis, properly selected convergence metrics on $\theta_k$ and $\omega_k$ evolve as $x_k$ and $y_k$ above, respectively, according to \eqref{lem:lyapunov:sc:def} for strongly convex and P\L~functions and \eqref{lem:lyapunov:def} for non-convex functions, while the sequences $\{a_k,\, b_k,\,c_k,\,d_k,\,e_k,\,f_k\}$ are ratios and products of the step sizes $\{\alpha_k\}$ and $\{\beta_k\}$.\looseness=-1






==> old_files/Dec1_2022_combinelambda/proof_mainresults.tex <==
\subsection{Proof of Main Results}\label{sec:proof_mainresults}

In this section, we present the proof of Theorem~\ref{thm:convergence_decision_pl} which considers functions observing the P\L~condition. The analyses of strongly convex and general non-convex functions use similar techniques: one needs to properly select a convergence metric according to the function structure, set up a step-wise decay of the convergence metric like Proposition~\ref{prop:pl_nonconvex} which forms a coupled dynamical system with Proposition~\ref{prop:auxiliary}, and apply the two-time-scale lemma introduced in Section~\ref{sec:lyapunov_lemma} to the coupled system. The detailed proofs of Theorems~\ref{thm:convergence_decision_sc} and \ref{thm:convergence_decision_nonconvex} can be found in our companion paper \cite{zeng2021two}.


From the analysis of the auxiliary variable in Proposition \ref{prop:auxiliary}, we have for all $k\geq\Kcal$
\begin{align*}
    \mathbb{E}[\|z_{k+1}\|^2] &\leq (1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_G\beta_k}{2})\mathbb{E}[\|z_{k}\|^2]\hspace{-2pt}+\hspace{-2pt}C_2\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}+C_2\tau_k^2\beta_{k-\tau_k}\beta_k.
\end{align*}
Due to the boundedness of the operator $H$,
\begin{align*}
    \|\theta_k\|\leq \|\theta_0\|+\sum_{t=0}^{k-1}\|\theta_{t+1}-\theta_t\|\leq \|\theta_0\|+\sum_{t=0}^{k-1}\frac{B \alpha}{t+1}\leq\|\theta_0\|+\frac{B \alpha\log(k+1)}{\log(2)},
\end{align*}
where the last inequality follows from $\sum_{t=0}^{t'}\frac{1}{(t+1)^{u}}\leq \frac{\log(t'+2)}{\log(2)}$ for any $t'\geq 0$. This relation implies for any $k\geq 0$
\begin{align*}
    \|\theta_k\|^2\leq 2\|\theta_0\|^2+\frac{2B^2 \alpha^2 \log^2(k+1)}{\log^2(2)}\leq 24(\|\theta_0\|^2+B^2 \alpha^2)\log^2(k+1).
\end{align*}
Using this inequality in the bound on $\mathbb{E}[\|z_{k+1}\|^2]$, we have
\begin{align*}
    \mathbb{E}[\|z_{k+1}\|^2]&\leq (1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_G\beta_k}{2})\mathbb{E}[\|z_{k}\|^2]\hspace{-2pt}+\hspace{-2pt}C_2\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}\hspace{-2pt}+\hspace{-2pt}C_2\tau_k^2\beta_{k-\tau_k}\beta_k\notag\\
    % &\leq \hspace{-2pt}(1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_G\beta_k}{2})\mathbb{E}[\|z_{k}\|^2]\hspace{-2pt}+\hspace{-2pt}24C_2(\|\theta_0\|^2\hspace{-2pt}+\hspace{-2pt}B^2 \alpha^2)\tau_k^2\beta_{k-\tau_k}\beta_k\log^2(k+1)\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}\hspace{-2pt}+\hspace{-2pt}C_2\tau_k^2\beta_{k-\tau_k}\beta_k\notag\\
    &\hspace{-20pt}\leq \hspace{-2pt}(1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_G\beta_k}{2})\mathbb{E}[\|z_{k}\|^2]\hspace{-2pt}+\hspace{-2pt}24C_2 (\|\theta_0\|^2\hspace{-2pt}+\hspace{-2pt}B^2 \alpha^2\hspace{-2pt}+\hspace{-2pt}1)\tau_k^2\beta_{k-\tau_k}\beta_k\log^2(k\hspace{-2pt}+\hspace{-2pt}1)\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}.
\end{align*}
% where in the last inequality simply re-combines the terms.


We can apply Lemma \ref{lem:lyapunov} case 1) to the result of Proposition~\ref{prop:pl_nonconvex} and the inequality above with $\tau=\Kcal$ and
\begin{align*}
    & x_k\hspace{-2pt}=\hspace{-2pt}\mathbb{E}[f(\theta_{k})\hspace{-2pt}-\hspace{-2pt}f^{\star}],\,\, y_k\hspace{-2pt}=\hspace{-2pt}\mathbb{E}\left[\|z_k\|^2\right],\,\, a_k\hspace{-2pt}=\hspace{-2pt}\lambda_f \alpha_k,\,\, b_k\hspace{-2pt}=\hspace{-2pt}\frac{L^2\alpha_k}{2},\,\, c_k\hspace{-2pt}=\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k},\\
    & d_k=\frac{\lambda_G \beta_k}{2},\,\,e_k=0,\,\, f_k=24C_2 (\|\theta_0\|^2\hspace{-2pt}+\hspace{-2pt}B^2 \alpha^2\hspace{-2pt}+\hspace{-2pt}1)\tau_k^2\beta_{k-\tau_k}\beta_k\log^2(k\hspace{-2pt}+\hspace{-2pt}1)+\frac{2L^2 B^2 \alpha_k^2}{\lambda_G\beta_k}.
\end{align*}
In this case, one can verify that we can choose $A=\frac{L^2}{\lambda_f}$ if the step size sequences satisfy $\frac{\alpha_k}{\beta_k}\leq\frac{\lambda_G}{4\lambda_f}$.
As a result of Lemma \ref{lem:lyapunov} case 1), we have for all $k\geq\Kcal$\vspace{-8pt}
\begin{align*}
    \mathbb{E}\left[f(\theta_{k})\hspace{-2pt}-\hspace{-2pt}f^{\star}\right]\hspace{-2pt}&\leq\hspace{-2pt} \left(\mathbb{E}\big[f(\theta_{\Kcal})-f^{\star}\right]+\frac{2L^{2} \alpha_{\Kcal}}{\lambda_{G} \beta_{\Kcal}}\mathbb{E}[\|z_{\Kcal}\|^2]\big)\hspace{-2pt}\prod_{t=\Kcal}^{k-1}\hspace{-2pt}(1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_f \alpha_t}{2})\hspace{-2pt}+\hspace{-2pt}\sum_{\ell=\Kcal}^{k-1}\prod_{t=\ell+1}^{k-1}(1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_f \alpha_t}{2})\notag\\
    &\hspace{-42pt}\times\Big(\frac{25L^2B^3}{2}\tau_k^2\alpha_{\ell}\alpha_{\ell-\tau_k}\hspace{-4pt}+\hspace{-3pt}\frac{48C_2 L^2}{\lambda_G} (\|\theta_0\|^2\hspace{-3pt}+\hspace{-3pt}B^2\hspace{-1pt} \alpha^2\hspace{-3pt}+\hspace{-3pt}1)\tau_k^2\beta_{k-\tau_k}\alpha_k\hspace{-1pt}\log^2\hspace{-1pt}(k\hspace{-3pt}+\hspace{-3pt}1)\hspace{-2pt}+\hspace{-2pt}\frac{4L^4 B^2 \alpha_k^3}{\lambda_G^2\beta_k^2}\Big).
\end{align*}
Plugging in the step sizes to the second term, we have
\begin{align}
    \mathbb{E}\left[f(\theta_{k})-f^{\star}\right]&\leq \left(\mathbb{E}\left[f(\theta_{\Kcal})-f^{\star}\right]+\frac{2L^{2} \alpha_{\tau_k}}{\lambda_{G} \beta_{\tau_k}}\mathbb{E}[\|z_{\Kcal}\|^2]\right)\prod_{t=\Kcal}^{k-1}(1-\frac{\lambda_f \alpha_t}{2})\notag\\
    &\hspace{10pt}+\tau_k^2\sum_{\ell=\Kcal}^{k-1}\Big(\frac{25L^2B^3\alpha_0^2}{2c_{\tau}(\ell+1)^2}+\frac{4L^4 B^2 \alpha_0^3}{\lambda_G^2 \beta_0^2 (\ell+1)^{5/3}}\notag\\
    &\hspace{20pt}+\hspace{-2pt}\frac{48C_2 L^2}{\lambda_G} (\|\theta_0\|^2\hspace{-2pt}+\hspace{-2pt}B^2 \alpha_0^2\hspace{-2pt}+\hspace{-2pt}1)\frac{\alpha_0\beta_0}{c_{\tau}(\ell+1)^{5/3}}\log^2(k\hspace{-2pt}+\hspace{-2pt}1)\Big)\hspace{-4pt} \prod_{t=\ell+1}^{k-1}\hspace{-4pt}(1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda_f \alpha_t}{2})\notag\\
    &\leq \left(\mathbb{E}\left[f(\theta_{\Kcal})-f^{\star}\right]+\frac{2L^{2} \alpha_{\Kcal}}{\lambda_{G} \beta_{\Kcal}}\mathbb{E}[\|z_{\Kcal}\|^2]\right)\prod_{t=\Kcal}^{k-1}(1-\frac{\lambda_f \alpha_t}{2})\notag\\
    &\hspace{10pt}+\tau_k^2\log^2(k+1)\sum_{\ell=\Kcal}^{k-1}\frac{C_3}{(\ell+1)^{5/3}} \prod_{t=\ell+1}^{k-1}(1-\frac{\lambda_f \alpha_t}{2}),
    \label{thm:convergence_decision_pl:eq2.6}
\end{align}
where we use the fact that $\frac{1}{\log^2(k+1)}\leq 12$ for all $k>0$ and the definition of $C_3$.

Since $1+c\leq\exp(c)$ for any scalar $c$, we have
\begin{align}
    \prod_{t=\Kcal}^{k-1}(1-\frac{\lambda_f \alpha_t}{2})&\leq \prod_{t=\Kcal}^{k-1}\exp(-\frac{\lambda_f \alpha_t}{2})=\exp(-\sum_{t=\Kcal}^{k-1}\frac{\lambda_f \alpha_t}{2})\leq \exp(-\frac{\lambda_f \alpha_0}{2}\sum_{t=\Kcal}^{k-1}\frac{1}{t+1})\notag\\
    &\leq \exp(-\frac{\lambda_f \alpha_0}{2}\log(\frac{k+1}{\Kcal+1}))\leq(\frac{\Kcal+1}{k+1})^{\frac{\lambda_f \alpha_0}{2}}\leq \frac{\Kcal+1}{k+1},
    \label{thm:convergence_decision_pl:eq2.7}
\end{align}
where the last inequality results from $\alpha_0\geq\frac{2}{\lambda_f}$, and the third inequality follows from $\sum_{t=k_1}^{k_2}\frac{1}{t+1}\geq \log(\frac{k_2+2}{k_1+1})$.
Similarly, we have
\begin{align}
    \prod_{t=\ell+1}^{k-1}(1-\frac{\lambda_f \alpha_t}{2})\leq \frac{2\ell+1}{k+1}\leq \frac{2(\ell+1)}{k+1}.
    \label{thm:convergence_decision_pl:eq2.8}
\end{align}
Using \eqref{thm:convergence_decision_pl:eq2.7} and \eqref{thm:convergence_decision_pl:eq2.8} in \eqref{thm:convergence_decision_pl:eq2.6}, \begin{align*}
    \mathbb{E}\left[f(\theta_{k})-f^{\star}\right]&\leq \left(\hspace{-2pt}\mathbb{E}\left[f(\theta_{\Kcal})\hspace{-2pt}-\hspace{-2pt}f^{\star}\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^{2} \alpha_{\Kcal}}{\lambda_{G} \beta_{\Kcal}}\mathbb{E}[\|z_{\Kcal}\|^2]\hspace{-2pt}\right)\hspace{-2pt}\frac{\Kcal}{k\hspace{-2pt}+\hspace{-2pt}1}\hspace{-2pt}+\hspace{-2pt}\frac{\log^2(k\hspace{-2pt}+\hspace{-2pt}1)\tau_k^2}{k+1} \hspace{-3pt}\sum_{\ell=\Kcal}^{k-1}\hspace{-4pt}\frac{2C_3}{(\ell\hspace{-2pt}+\hspace{-2pt}1)^{2/3}}\notag\\
    &\leq\frac{\Kcal+1}{k+1}\left(\mathbb{E}\left[f(\theta_{\Kcal})-f^{\star}\right]+\frac{2L^{2} \alpha_0}{\lambda_{G} \beta_0}\mathbb{E}[\|z_{\Kcal}\|^2]\right)+\frac{2C_3\log^2(k+1)\tau_k^2}{3(k+1)^{2/3}},
%    \label{thm:convergence_decision_pl:eq2.95}
\end{align*}
where the second inequality is a result of the relation $\sum_{t=0}^{t'}\frac{1}{(t+1)^{2/3}}\leq\frac{(t'+1)^{1/3}}{3}$ for any $t'\geq0$. The claimed result follows from this and \eqref{assump:mixing:tau}.


% \qed


==> old_files/Dec1_2022_reviseproofsketch/Analysis_Theorems.tex <==

\section{Main Results}\label{sec:main_results}
In Section~\ref{subsec:main_theorems}, we present the main results of this paper, which are the finite-time convergence of Algorithm \ref{Alg:two-time-scale-SGD} under different function structure. Then, we briefly explain the main technical challenges and the complex coupling of the decision variable, auxiliary variable, and time-varying Markovian samples in Section \ref{subsec:tech_challenges}. 
% We then state the convergence of the auxiliary variable in Section \ref{subsec:conv_auxiliary}, which is an important step towards deriving the convergence of the decision variable.
In Section \ref{sec:lyapunov_lemma}, we introduce an important lemma that performs Lyapunov analysis on a coupled dynamical system of two inequalities. This lemma is a unified tool to analyze our algorithm under different function structures and may be of independent interest in the study of the finite-time performance of multiple-time-scale dynamical systems apart from those considered in this paper. Finally, we prove the theorem under the P\L~condition in Section~\ref{sec:proof_mainresults}. Strongly convex and general non-convex functions can be treated with similar analytical techniques, and the full details of their analyses can be found in the companion paper \cite{zeng2021two}.


\subsection{Finite-Time Complexity of Two-Time-Scale SGD}\label{subsec:main_theorems}
This subsection establishes the finite-time complexity of the two-time-scale SGD algorithm under four structural properties of the objective function, namely, strong convexity,
non-convexity with the P\L~condition, and general non-convexity. Our results are derived under the assumptions introduced in Section \ref{sec:assumptions}, which we assume always hold in the rest of this paper.


The convergence of Algorithm \ref{Alg:two-time-scale-SGD} relies on $\alpha_k,\beta_k\rightarrow 0$ with reasonable rates. As mentioned in Section \ref{sec:two-time-scale-SGD}, $\alpha_{k}$ needs to be much smaller than $\beta_{k}$ to approximate the nested-loop algorithm where multiples auxiliary variable updates are performed for each decision variable update. Therefore, we consider the following choices of step sizes\looseness=-1
\begin{align}
    \alpha_k = \frac{\alpha_0}{(k+1)^{a}}, \quad \beta_k = \frac{\beta_0}{(k+1)^{b}},\quad\forall k\geq 0,\label{stepsizes}
\end{align}
where $a,b,\alpha_0,\beta_0$ are some constants satisfying $0 < b\leq a\leq 1$ and $0< \alpha_0 \leq  \beta_0$. 
Given $\alpha_{k}$, recall from Definition \ref{def:mixing_time} that  $\tau(\alpha_{k})$ is the mixing time associated with $\alpha_{k}$. In the sequel, for convenience we denote $\tau_{k}\triangleq\tau(\alpha_k)$.
Since $\tau_{k} \leq C\log((k+1)^{a}/\alpha_0)$ (from \eqref{assump:mixing:tau}), we have
$\lim_{k\rightarrow\infty}\alpha_{k}\tau_{k}^2 = \lim_{k\rightarrow\infty}\beta_{k}\tau_{k}^2 = 0$.
This implies that there exists a positive integer $\Kcal$ such that
\begin{align}
    \beta_{k-\tau_k}\tau_k^2\leq\min\Big\{1,\frac{1}{6LB},\frac{\lambda}{22C_1+32D^2},\frac{\lambda}{2C_2},\frac{\lambda^3}{32L^2 C_2}\Big\},\quad\forall k\geq\Kcal,\label{notation:Kcal}
\end{align}
where $C_1$ and $C_2$ are positive constants defined as 
\begin{align}
C_1 &= 18D^2+20LDB,\,\,C_2=(4D^2+1)(4C_1+32D^2)+\frac{2L^2 B^2}{\lambda}+2L^2 B^2.
\label{notation:constant_C}
\end{align}
% 
In addition, there exists a constant $c_{\tau}\in(0,1)$ such that for any $k>\tau_k$ we have
\begin{align}
    \tau_k\leq(1-c_{\tau})k+(1-c_{\tau}), \quad\text{and}\quad c_{\tau}(k+1)\leq k-\tau_k+1\leq k+1.
\end{align}

We carefully come up with the constants and conditions in \eqref{notation:Kcal} and \eqref{notation:constant_C} to prevent an excessively large step size from destroying the stability of the updates. {\color{red}We note that $\Kcal$ is a constant that only depends on the quantities involved in the step sizes in \eqref{stepsizes}.}


\subsubsection{Strong Convexity} We consider the following assumption on function $f$. 

\begin{assump}\label{assump:sc}
The function $f$ is strongly convex with constant $\lambda$\footnote{\color{red}Without any loss of generality, we slightly overload $\lambda$, the strong monotonicity constant of the operator $G$ in Assumption~\ref{assump:stronglymonotone_G},
to denote the strong convexity constant here.}
\begin{align}
    f(y) \geq f(x)+\langle\nabla f(x),y-x\rangle+\frac{\lambda}{2}\|y-x\|^{2}, \quad \forall x,y\in\mathbb{R}^d.\label{assump:sc:ineq}
\end{align}
\end{assump}
% Our first main result shows that when $f$ is strongly convex, the iterates of Algorithm~\ref{Alg:two-time-scale-SGD} converge to the optimal solution at a rate $\widetilde{\Ocal}(k^{-2/3})$ up to a logarithm factor.
\begin{thm}[Strongly Convex]
Suppose that Assumption \ref{assump:sc} holds.
Let the step size sequences $\{\alpha_k\}$ and $\{\beta_k\}$ satisfy \eqref{stepsizes} with
\begin{align*}
a=1,\quad b=2/3,\quad \alpha_0\geq \frac{4}{\lambda},\quad\text{and}\quad \frac{\alpha_0}{\beta_0}\leq\frac{1}{2}\cdot
\end{align*}
Then for all $k\geq \Kcal$ where $\Kcal$ is defined in \eqref{notation:Kcal},
% (again, we note that $\Kcal$ is a constant depending only on $a,b,\alpha_0,\beta_0$ and the structures of the function $f$),
we have
\begin{align*}
    \mathbb{E}\left[\|\theta_k-\theta^{\star}\|^2\right]
    &\leq \frac{\Kcal+1}{k+1}\left(\mathbb{E}\left[\|\theta_{\Kcal}-\theta^{\star}\|^2\right]+\frac{4 L^{2} \alpha_0}{\lambda^2 \beta_0}\mathbb{E}[\|\omega_{\Kcal}-\omega^{\star}(\theta_{\Kcal})\|^2]\right)\notag\\
    &\hspace{-43pt}+\frac{C^2\log^2((k+1)/\alpha_0)}{3(k+1)^{2/3}}\left((6C_2+2B^2+\frac{8L^2 C_2}{\lambda^2}(2\|\theta^{\star}\|^2+1))\frac{\alpha_0\beta_0}{c_{\tau}}+\frac{16L^4 B^2 \alpha_0^3}{\lambda^3 \beta_0^2}\right).
    % \label{thm:convergence_decision_sc:ineq}
\end{align*}
\label{thm:convergence_decision_sc}
\end{thm}
% \begin{remark}
% Then the iterates $\theta_k$ converge to the unique optimal solution $\theta^{\star}$ at a rate of $\Ocal((k+1)^{-2/3})$ under the choice of step size $a=1$ and $b=2/3$. Compared with the standard SGD where a convergence rate of $\Ocal((k+1)^{-1})$ is achieved for strongly convex functions, the two-time-scale algorithm is slower by $\Ocal((k+1)^{1/3})$ due to the online update of the auxiliary variable.
{\color{red}
Our theorem states that when $f$ is strongly convex the iterates of Algorithm~\ref{Alg:two-time-scale-SGD} converge to the optimal solution with rate $\widetilde{\Ocal}(k^{-2/3})$.
Comparing with the deterministic gradient descent setting where the convergence rate is linear and the standard SGD setting where the convergence rate is $\Ocal(k^{-1})$, our result reflects the compromise in the convergence rate due to the gradient noise and inaccurate auxiliary variable.
Compared with the convergence rate of the two-time-scale SA algorithm for bi-level optimization \cite{hong2020two} under i.i.d. samples, our rate is the same up to a logarithm factor which naturally arises from the bias caused by the time-varying Markovian samples.
}
% We note that the rate in Theorem~\ref{thm:convergence_decision_sc} is similar to the one in two-time-scale SA studied in \cite{doan2021finite}. However, while \cite{doan2021finite} considers samples generated by a fixed Markov chain, the samples in our algorithm are generated by a time-varying Markov process parameterized by the decision variable. 
% \end{remark}


\subsubsection{Non-Convexity under P\L~Condition} 
We also study the convergence of Algorithm \ref{Alg:two-time-scale-SGD} under the following condition.
\begin{assump}\label{assump:PL_condition}
There exists a constant $\lambda>0$ such that
\[\frac{1}{2}\|\nabla f(x)\|^2 \geq \lambda \left(f(x)-f^{\star}\right), \quad \forall x\in\mathbb{R}^d.\]
\end{assump}
This is known as the P\L~condition and is introduced in \cite{polyak1987introduction,lojasiewicz1963topological}. The P\L~condition does not imply convexity, but guarantees the linear convergence of the objective function value when gradient descent is applied to solve a non-convex optimization problem \cite{karimi2016linear}, which resembles the convergence rate of gradient descent for strongly convex functions. Recently, this condition has been observed to hold in many important practical problems such as supervised learning with an over-parametrized neural network \cite{liu2020toward} and the linear quadratic regulator in optimal control \cite{fazel2018global,yang2019global}. 


\begin{thm}[P\L~Condition]\label{thm:convergence_decision_pl}
Suppose the function $f$ satisfies Assumption~\ref{assump:PL_condition}.
In addition, we assume that the stochastic gradient is bounded, i.e. there exists a constant $B>0$ such that \footnote{Again, for the convenience of notation, we use the same constant $B$ as in Assumption~\ref{assump:Lipschitz_omega}.}
\begin{align}
\|H(\theta,\omega,X)\| \leq B,\quad \forall \theta\in\Rset^{d}, \omega\in\Rset^{r},X\in\Xcal.    \label{assump:H_bounded}
\end{align}
Let the step size sequences $\{\alpha_k\}$ and $\{\beta_k\}$ satisfy \eqref{stepsizes} with
\begin{align*}
    a=1,\quad b=2/3,\quad\alpha_0\geq \max\{1,\frac{2}{\lambda}\},\quad\text{and}\quad\frac{\alpha_0}{\beta_0}\leq\frac{1}{4}.
\end{align*}
Then for all $k\geq \Kcal$ where $\Kcal$ is defined in \eqref{notation:Kcal}, we have
\begin{align*}
    \mathbb{E}\left[f(\theta_{k})\hspace{-2pt}-\hspace{-2pt}f^{\star}\right]&\hspace{-3pt}\leq\hspace{-3pt} \frac{\Kcal+1}{k+1}\hspace{-2pt}\left(\hspace{-2pt}\mathbb{E}\left[f(\theta_{\Kcal})\hspace{-2pt}-\hspace{-2pt}f^{\star}\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^{2} \alpha_0}{\lambda \beta_0}\mathbb{E}[\|\omega_{\Kcal}-\omega^{\star}(\theta_{\Kcal})\|^2]\hspace{-2pt}\right)\hspace{-2pt}+\hspace{-2pt}\frac{2C^2 C_3\log^4(k\hspace{-2pt}+\hspace{-2pt}1)}{3(k+1)^{2/3}},
\end{align*}
where $C_3=\frac{150L^2B^3\alpha_0^2}{c_{\tau}}+\frac{48L^2 C_2}{\lambda} (\|\theta_0\|^2+B^2 \alpha_0^2+1)\frac{\alpha_0\beta_0}{c_{\tau}}+\frac{48L^4 B^2 \alpha_0^3}{\lambda^2 \beta_0^2}$.
\end{thm}

{\color{red} Under the P\L~condition, we show that $f(\theta_k)$ converges to the optimal function value $f^{\star}$ with rate $\widetilde{\Ocal}(k^{-2/3})$. This is the same rate as if $f$ is strongly convex. However, in this case the convergence is measured in the function value, whereas under strong convexity the iterates $\theta_k$ converge to the unique global minimizer. The convergence rates of deterministic gradient descent and standard SGD under the P\L~condition also match those in the strongly convex case. To our best knowledge, functions exhibiting the P\L~condition have not been studied in the bi-level optimization framework.}




\subsubsection{Non-Convexity} 
Finally, we study the case where the objective function $f$ is non-convex and smooth. In general, we cannot find an optimal solution and may only reach a stationary point. 
Analyzing the convergence without any convexity or P\L~condition is more challenging, and we need to make an additional assumption to ensure stability. 
% This assumption replaces \eqref{assump:HG_smooth:ineq} in Assumption \ref{assump:HG_smooth}.

\begin{assump}\label{assump:HG_smooth_nonconvex}
There exists a constant $L > 0$ such that
\begin{align*}
    \left\|G(\theta_1,\omega_1,X)-G(\theta_2,\omega_2,X)\right\| \leq L(\|\omega_1-\omega_2\|+1),\forall \theta_{1},\theta_{2}\in\mathbb{R}^d,\omega_{1},\omega_{2}\in\mathbb{R}^r,X\in\Xcal.
\end{align*}
\end{assump}
We note that this assumption holds in the actor-critic algorithm we discuss in Section \ref{sec:MDP_AC} where $G$ does not depend on $\theta$, as well as in problems where $G$ is bounded in $\theta$.



\begin{thm}[Non-convex]\label{thm:convergence_decision_nonconvex}
% Choose $a=3/5$ and $b=2/5$. 
Let the step size $\{\alpha_k\}$ and $\{\beta_k\}$ satisfy \eqref{stepsizes} with
$a=3/5$, and $b=2/5$.
Under Assumptions \ref{assump:HG_smooth_nonconvex}, we have for all $k\geq\Kcal$
\begin{align*}
    \min_{t\leq k}\mathbb{E}[\|\nabla f(\theta_t)\|^2] &\leq \frac{4}{\alpha_0(k+1)^{2/5}}\mathbb{E}[f(\theta_{\Kcal})-f^{\star}]+\frac{4L^2}{\beta_0\lambda (k+1)^{2/5}}\mathbb{E}[\|\omega_{\Kcal}-\omega^{\star}(\theta_{\Kcal})\|^2]\notag\\
    &\hspace{15pt}+\left(\frac{25L^2B^3\alpha_0^2}{2c_{\tau}}+\frac{2L^4 B^2 \alpha_0^3}{\lambda \beta_0^2}+\frac{L^2 \alpha_0\beta_0 C_2}{c_{\tau}\lambda}\right)\frac{8\tau_k^2\log(k+1)}{5\log(2)c_{\tau}(k+1)^{2/5}}.
\end{align*}
\end{thm}

{\color{red} Our theorem in the non-convex case shows the convergence of the two-time-scale SGD algorithm to a stationary point of the objective function (measured by the squared norm of the gradient) with rate $\widetilde{\Ocal}(k^{-2/5})$.
One may contrast this with the convergence rate of deterministic gradient descent $\Ocal(k^{-1})$ and standard SGD $\Ocal(k^{-1/2})$ to see the cost of the gradient noise and auxiliary variable inaccuracy. Compared with the bi-level optimization algorithm under i.i.d. samples \cite{hong2020two}, our rate is again the same up to a logarithm factor due to the time-varying Markovian samples. 
}



\subsection{Technical Challenges \& Coupling between Decision and Auxiliary Variables}\label{subsec:tech_challenges}
The main technical challenge in analyzing Algorithm \ref{Alg:two-time-scale-SGD} is to handle the coupling between $\theta$, $\omega$,
% (two-time-scale updates) 
and the time-varying Markovian samples simultaneously. 
% It also worth noting that the Markovian samples affect the current update of $\theta$, which induces the Markov chain used to generate the future samples.
To illustrate the complications involved, we quickly look at how we might show $\|f(\theta_k)-f^{\star}\|^2\rightarrow 0$ in the case where $f$ observes the P\L~condition.
For the simplicity of notation, we define $z_k\triangleq\omega_k-\omega^{\star}(\theta_k)$ and
\begin{align}
\begin{aligned}
    &\widebar{\Delta H_{k}} \triangleq H(\theta_k,\omega_k,X_k)-H(\theta_k,\omega^{\star}(\theta_k),X_k)\\
    &\Delta H_k \triangleq H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\\
    &\Delta G_k \triangleq G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})].
    \end{aligned}
    \label{eq:Delta_z_def}
\end{align}
We can think of $\widebar{\Delta H_k}$ as the bias due to the inaccurate auxiliary variable and $\Delta H_{k}$ and $\Delta G_{k}$ as the errors that the Markovian samples cause to $H$ and $G$.


From the update rule \eqref{alg:update_theta} and the $L$-smoothness of the function $f$, we have 
\begin{align}
    &f(\theta_{k+1})\leq f(\theta_{k})+\langle\nabla f(\theta_k),\theta_{k+1}-\theta_k\rangle+\frac{L}{2}\|\theta_{k+1}-\theta_k\|^2\notag\\
    &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega_k,X_k)\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k,X_k)\|^2\notag\\
    % &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle\notag\\
    % &\hspace{20pt}-\alpha_k\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    &= f(\theta_{k})-\alpha_k\langle\nabla f(\theta_k),\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\notag\\
    &\hspace{20pt}-\alpha_k\left\langle\nabla f(\theta_k), \Delta H_k\hspace{-2pt}+\hspace{-2pt}\widebar{\Delta H_k}\right\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2\notag\\
    &= f(\theta_{k})\hspace{-2pt}-\hspace{-2pt}\alpha_k\|\nabla f(\theta_k)\|^2\hspace{-2pt}-\hspace{-2pt}\alpha_k\left\langle\nabla f(\theta_k), \Delta H_k\hspace{-2pt}+\hspace{-2pt}\widebar{\Delta H_k}\right\rangle+\frac{L \alpha_k^2}{2}\|H(\theta_k,\omega_k, X_k)\|^2,
    \label{prop:pl_nonconvex:eq1}
\end{align}
where the last equality follows from \eqref{operator:H}, i.e. $\nabla f(\theta_k)=\mathbb{E}_{\hat{X}\sim \mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]$. If the samples were i.i.d. and the auxiliary variables were always solved perfectly, we would have $\mathbb{E}[\Delta H_k]=\mathbb{E}[\widebar{\Delta H_k}]=0$, reducing the problem to the one studied in the standard SGD. The focus of our work is to investigate how the two terms can be properly controlled in the presence of the Markovian noise and inexact auxiliary variables. To analyze the term involving $\Delta H_k$ we leverage Assumptions \ref{assump:markov-chain} and \ref{assump:tv_bound}.
\begin{lem}
    For any $k\geq \tau_k$, we have
    \begin{align*}
    \mathbb{E}\left[-\left\langle\nabla f(\theta_k),\Delta H_k\right\rangle\right] &\leq 12L^2B^3\tau_k^2\alpha_{k-\tau_k}.
    \end{align*}
\label{lem:Gamma_bound}
\end{lem}
\begin{proof}
Our Markov process is a time-varying one (they depend on the iterates $\theta$). Therefore, one cannot directly utilize Assumption \ref{assump:markov-chain} to analyze the bias of $G$ in Algorithm \ref{Alg:two-time-scale-SGD} since the mixing time is defined for a fixed Markov chain (see Definition \ref{def:mixing_time}). To handle this difficulty, we introduce an auxiliary Markov chain $\{\widetilde{X}_{k}\}$ generated under the decision variable $\theta_{k-\tau_k}$ starting from $X_{k-\tau_{k}}$ as follows
\begin{align}
% X_{k-\tau_k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  
{X}_{k-\tau_k} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \widetilde{X}_{k-\tau_k+1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \cdots \widetilde{X}_{k-1} \stackrel{\theta_{k-\tau_k}}{\longrightarrow}  \widetilde{X}_{k}.
\label{eq:def_distribution_d}
\end{align}
% and we use $d_k$ to denote the distribution of $\widetilde{X}_{k}$. 
% Thus, one can apply Assumption \ref{assump:markov-chain} to $\{\widetilde{X}_{k}\}$. 
For clarity, we recall original the time-varying Markov processes $\{X_k\}$ generated by Algorithm~\ref{Alg:two-time-scale-SGD}
\begin{align*}
X_{k-\tau_k} \stackrel{\theta_{k-\tau_k+1}}{\longrightarrow} X_{k-\tau_k+1} \stackrel{\theta_{k-\tau_k+2}}{\longrightarrow} \cdots \stackrel{\theta_{k-1}}{\longrightarrow} X_{k-1} \stackrel{\theta_{k}}{\longrightarrow} X_{k}.
\end{align*}
Using the shorthand notation $y_k=\nabla f(\theta_k)$, we define the following quantities
\begin{align*}
    &T_1 = \mathbb{E}[\langle y_k-y_{k-\tau_k},\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]-H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle]\notag\\
    &T_2 = \mathbb{E}[\langle y_{k-\tau_k},H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)-H(\theta_k,\omega^{\star}(\theta_k),X_k)\rangle]\notag\\
    &T_3 = \mathbb{E}[\langle y_{k-\tau_k},H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\rangle]\notag\\
    &T_4 = \mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-2pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\bar{X})]-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\rangle]\notag\\
    &T_5 = \mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\hat{X})]\hspace{-2pt}-\hspace{-2pt}\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-4pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\bar{X})]\rangle]\notag\\
    &T_6 = \mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hat{X}]\rangle].
\end{align*}
It is easy to see that
\begin{align}
    -\mathbb{E}\left[\left\langle\nabla f(\theta_k),\Delta H_k\right\rangle\right]
    % &=-\mathbb{E}\big[\langle \nabla f(\theta_k),H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\big]\notag\\
    % &=-\mathbb{E}\big[\langle \nabla f(\theta_k)-\nabla f(\theta_{k-\tau_k}),H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\big]\notag\\
    % &\hspace{20pt}-\mathbb{E}\big[\langle \nabla f(\theta_{k-\tau_k}),H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\rangle\big]\notag\\
    &=T_1+T_2+T_3+T_4+T_5+T_6.
    \label{eq:bound_Gamma_breakdown}
\end{align}
We analyze the terms of \eqref{eq:bound_Gamma_breakdown} individually. First, we treat $T_1$ using the boundedness of $H$ and the Lipschitz continuity of $\nabla f$
\begin{align}
T_1&\leq \mathbb{E}\big[\left\|y_k-y_{k-\tau_k}\right\|\left\|H(\theta_k,\omega^{\star}(\theta_k),X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})]\right\|\big]\notag\\
&\leq L\mathbb{E}\big[\left\|\theta_k-\theta_{k-\tau_k}\right\|\big]]\cdot 2B\leq2B^2 L\tau_k\alpha_{k-\tau_k},
\label{lem:Gamma_bound:T1}
\end{align}
where the last inequality follows from
\[\|\theta_k-\theta_{k-\tau_k}\|\leq\sum_{t=k-\tau_k}^{k}\|\alpha_t H(\theta_t,\omega_t,X_t)\|\leq B\tau_k\alpha_{k-\tau_k}.\]
% To bound $T_2$, we employ the boundedness $\nabla f$ and the Lipschitz continuity of $H$
Similarly, for $T_2$ we have
\begin{align}
    T_2&\leq \mathbb{E}\big[\|y_{k-\tau_k}\|\|H(\theta_k,\omega^{\star}(\theta_k),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\|\big]\notag\\
    &\leq B\mathbb{E}\big[\|H(\theta_k,\omega^{\star}(\theta_k),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\|\big]\notag\\
    &\leq BL\mathbb{E}\big[\|\theta_k-\theta_{k-\tau_k}\|+\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k-\tau_k})\|\big]\notag\\
    &\leq BL(L+1)\mathbb{E}\big[\|\theta_k-\theta_{k-\tau_k}\|\big]\leq B^2 L(L+1)\tau_k\alpha_{k-\tau_k}.
    \label{lem:Gamma_bound:T2}
\end{align}
To analyze $T_3$, we utilize the law of total expectation: given $\Fcal\subseteq\Fcal'$ and a random variable $X$ we have $\Eset[X\mid\Fcal] = \Eset[\Eset[X\mid\Fcal']\mid\Fcal]$.   

Let $\Fcal_k$ be $\Fcal_k=\{X_0,\ldots,X_k,\theta_0,\ldots,\theta_k,\omega_0,...,\omega_k\}$,
and for convenience we denote
\[p_{k}(x) = P(X_{k} = x\mid\Fcal_{k-1})\quad  \text{and}\quad  \tilde{p}_{k}(x) = P(\widetilde{X}_{k} = x\mid\Fcal_{k-1}).\]
Then, we have
\begin{align*}
    &\mathbb{E}\big[\left\langle y_{k-\tau_k},H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\right\rangle\mid \Fcal_{k-\tau_k}\big]\notag\\
    % &=\langle \nabla f(\theta_{k-\tau_k}),\mathbb{E}\big[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)\mid \Fcal_{k-\tau_k}\big]\rangle\notag\\
    &\leq\left\| y_{k-\tau_k}\right\|\|\mathbb{E}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\mid \Fcal_{k-\tau_k}]\|\notag\\
    &=\left\|y_{k-\tau_k}\right\|\big\|\mathbb{E}\big[\mathbb{E}\big[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),X_k)-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\hspace{-2pt}\mid\hspace{-2pt} \Fcal_{k-1}\big]\mid \Fcal_{k-\tau_k}\big]\big\|\notag\\
    &\leq B\mathbb{E}[\int_{\Xcal}H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),x)(p_k(x)-\widetilde{p}_k(x)) dx \mid \Fcal_{k-\tau_k}]\notag\\
    &\leq 2B^2 \mathbb{E}[d_{TV}(p_k(\cdot), \widetilde{p}_k(\cdot))\mid \Fcal_{k-\tau_k}]\notag\\
    &\leq 2B^2 \mathbb{E}\big[d_{TV}(p_{k-1}(\cdot),\widetilde{p}_{k-1}(\cdot))+L\|\theta_k-\theta_{k-\tau_k}\|\mid \Fcal_{k-\tau_k}\big],
\end{align*}
where the second inequality uses the definition of the TV distance in \eqref{eq:TV_def}, and the last inequality is a result of Assumption \ref{assump:tv_bound}. Recursively applying this inequality and taking the expectation, we get
\begin{align}
    T_3
    % &\leq 2B^2 \mathbb{E}\big[d_{TV}(p_{k-1}(\cdot),\widetilde{p}_{k-1}(\cdot))+L\|\theta_k-\theta_{k-\tau_k}\|\big]\notag\\
    &\leq 2B^2 L\sum_{t=k-\tau_k+1}^{k-1}\mathbb{E}[\|\theta_t-\theta_{k-\tau_k}\|]\leq 2B^3 L\tau_k^2\alpha_{k-\tau_k}.
    \label{lem:Gamma_bound:T3}
\end{align}
Similarly, to bound $T_4$, we again use the definition of TV distance
\begin{align*}
    &\mathbb{E}[\langle y_{k-\tau_k},\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\bar{X})]-H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)\rangle\mid\Fcal_{k-\tau_k}]\notag\\
    &\leq\left\|y_{k-\tau_k}\right\|\big\|\mathbb{E}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\widetilde{X}_k)-\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-2pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\bar{X})]\hspace{-2pt}\mid\hspace{-2pt}\Fcal_{k-\tau_k}]\big\|\notag\\
    &\leq B\cdot 2B \mathbb{E}[d_{TV}(\widetilde{p}_k(\cdot),\mu_{\theta_{k-\tau_k}})\mid \Fcal_{k-\tau_k}].
\end{align*}
Taking the expectation and using the definition of the mixing time \eqref{def:mixing_time},
\begin{align}
    T_4&\leq 2B^2 \mathbb{E}[d_{TV}(P(\widetilde{X}_k=\cdot),\mu_{\theta_{k-\tau_k}})]
    % \leq 2B^2 m\rho^{\tau_k}
    \leq 2B^2\alpha_k.
    \label{lem:Gamma_bound:T4}
\end{align}
We next consider $T_5$
\begin{align*}
    &\mathbb{E}[\langle y_{k-\tau_k},\hspace{-1pt}\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}\hspace{-1pt}(\theta_{k-\tau_k}),\hspace{-1pt}\hat{X})]\hspace{-2pt}-\hspace{-2pt}\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-6pt}[H(\theta_{k-\tau_k},\hspace{-1pt}\omega^{\star}\hspace{-1pt}(\theta_{k-\tau_k}),\hspace{-1pt}\bar{X})]\rangle\hspace{-2pt}\mid\hspace{-2pt}\Fcal_{k-\tau_k}]\notag\\
    &\leq B\|\mathbb{E}[\mathbb{E}_{\bar{X}\sim\mu_{\theta_{k-\tau_k}}}\hspace{-4pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\bar{X})]\hspace{-2pt}-\hspace{-2pt}\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\hspace{-2pt}[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hspace{-1pt}\hat{X})]\hspace{-2pt}\mid\hspace{-2pt}\Fcal_{k-\tau_k}]\|\notag\\
    &\leq 2B^2\mathbb{E}[d_{TV}(\mu_{\theta_{k-\tau_k}},\mu_{\theta_k})\mid \Fcal_{k-\tau_k}],
\end{align*}
where the last inequality again comes from the definition of the TV distance in \eqref{eq:TV_def}. By \eqref{assump:tv_bound:eq2} in Assumption \ref{assump:tv_bound}, we have
\begin{align}
    T_5&\leq2B^2\mathbb{E}[d_{TV}(\mu_{\theta_{k-\tau_k}},\mu_{\theta_k})]\leq 2B^2 L\mathbb{E}[\|\theta_k-\theta_{k-\tau_k}\|]\leq 2B^3 L\tau_k\alpha_k.
    \label{lem:Gamma_bound:T5}
\end{align}
Finally, we bound $T_6$ using the boundedness of $\nabla f$ and the Lipschitz continuity of $H$
\begin{align*}
    &T_6\leq \mathbb{E}\big[\| y_{k-\tau_k}\|\|\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}\big[H(\theta_{k-\tau_k},\omega^{\star}(\theta_{k-\tau_k}),\hat{X})\big]-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}\big[H(\theta_k,\omega^{\star}(\theta_k),\hat{X})\big]\big]\|\notag\\
    &\leq B L\mathbb{E}[\|\theta_{k-\tau_k}\hspace{-2pt}-\hspace{-2pt}\theta_k\|\hspace{-2pt}+\hspace{-2pt}\|\omega^{\star}(\theta_{k-\tau_k})\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_k)\|]\leq 2L^2B \mathbb{E}[\|\theta_{k-\tau_k}\hspace{-2pt}-\hspace{-2pt}\theta_k\|]\leq 2L^2B^2\tau_k\alpha_{k-\tau_k}.
    % \label{lem:Gamma_bound:T6}
\end{align*}
The claimed result follows from plugging the bounds on $T_1$-$T_6$ into \eqref{eq:bound_Gamma_breakdown}.
\end{proof}



In addition, we can use the Lipschitz continuity of $H$ to study the error caused by $\widebar{\Delta H_k}$ and show that it can be bounded by the sum of $\|\theta_k-\theta^{\star}\|^2$ and $\|z_k\|^2$. This bound on $\widebar{\Delta H_k}$ together with the bound on $\Delta H_k$ established in Lemma~\ref{lem:Gamma_bound} leads to the following proposition on the step-wise convergence of $\mathbb{E}[f(\theta_{k})-f^{\star}]$.
\begin{prop}\label{prop:pl_nonconvex}
Under Assumptions \ref{assump:HG_smooth}-\ref{assump:tv_bound}, we have for all $k\geq\Kcal$
\begin{align*}
    \mathbb{E}[f(\theta_{k+1})-f^{\star}]\leq (1\hspace{-2pt}-\hspace{-2pt}\lambda\alpha_k)\mathbb{E}[f(\theta_{k})-f^{\star}]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k}.
\end{align*}
\end{prop}
\begin{proof}
% We introduce the following technical lemma that bounds the a cross-term related to $\Delta H_k$. We skip the proof of Lemma~\ref{lem:Gamma_bound} due to its similarity to a lemma that we will later introduce and prove.

By the Lipschitz condition of the operator $H$,
\begin{align*}
    -\mathbb{E}[\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle] &\leq\frac{1}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2+\|H(\theta_k, \omega_k, X_k)-H(\theta_k, \omega^{\star}(\theta_k), X_k)\|^2]\notag\\
    &\leq\frac{1}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2}{2}\mathbb{E}\left[\|z_k\|^2\right].
\end{align*}
% \begin{align*}
%     \left\|\widebar{\Delta H_k}\right\|&=\left\|H(\theta_k, \omega_k, X_k)-H(\theta_k, \omega^{\star}(\theta_k), X_k)\right\|\leq L\left\|z_k\right\|,
% \end{align*}
% which implies
% \begin{align*}
%     -\mathbb{E}[\langle\nabla f(\theta_k),\widebar{\Delta H_k}\rangle] &\leq\frac{1}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2}{2}\mathbb{E}\left[\|z_k\|^2\right].
% \end{align*}
Using this inequality along with Lemma \ref{lem:Gamma_bound} in \eqref{prop:pl_nonconvex:eq1}, we have for all $k\geq \tau_k$ 
\begin{align*}
    \mathbb{E}[f(\theta_{k+1})]&\leq \mathbb{E}[f(\theta_{k})]-\alpha_k\left\langle\nabla f(\theta_k), \Delta H_k\right\rangle-\alpha_k\mathbb{E}[\|\nabla f(\theta_k)\|^2]\notag\\
    &\hspace{20pt}-\alpha_k\mathbb{E}\left[\left\langle\nabla f(\theta_k), \widebar{\Delta H_k}\right\rangle\right]+\frac{L B^2\alpha_k^2}{2}\notag\\
    &\leq \mathbb{E}[f(\theta_{k})]+12L^2B^3\tau_k^2\alpha_k\alpha_{k-\tau_k}-\alpha_k\mathbb{E}[\|\nabla f(\theta_k)\|^2]\notag\\
    &\hspace{20pt}+ \frac{\alpha_k}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{L B^2 \alpha_k^2}{2}\notag\\
    &\leq \mathbb{E}[f(\theta_{k})]-\frac{\alpha_k}{2}\mathbb{E}[\|\nabla f(\theta_k)\|^2]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k}\notag\\
    &\leq \mathbb{E}[f(\theta_{k})]-\lambda\alpha_k\mathbb{E}\left[f(\theta_k)-f^{\star}\right]+\frac{L^2\alpha_k}{2}\mathbb{E}\left[\|z_k\|^2\right]+\frac{25L^2B^3}{2}\tau_k^2\alpha_k\alpha_{k-\tau_k},
\end{align*}
where the last inequality is due to the P\L~condition.
Subtracting $f^{\star}$ from both sides of the inequality leads to the claimed result.
\end{proof}


Proposition~\ref{prop:pl_nonconvex} shows how the convergence of the decision variable depends on the precision of the auxiliary variable. We next aim to study how auxiliary variable evolves. Due to the assumption that the operator $H$ is bounded, the difference between $\theta_k$ and $\theta_{k-\tau_k}$ can be easily controlled by $\alpha_{k-\tau_k}$. However, the operator $G$ may not be bounded, and to properly handle $\|\omega_k-\omega_{k-\tau_k}\|$ we introduce the following lemma.
\begin{lem}\label{lem:omega_k-omega_k-tau}
For all $k\geq\tau_k$, we have 
\begin{align*}
\|\omega_k-\omega_{k-\tau_k}\|&\leq 3D\beta_{k-\tau_k}\tau_k\left(\|\omega_{k}\| +\|\theta_{k}\|+1\right).
% \notag\\
% &\leq \frac{1}{2}\left(\|\omega_{k}\| +\|\theta_{k}\|+1\right),
\end{align*}
% and
% \begin{align*}
%     \|\omega_k-\omega_{k-\tau_k}\|^2\leq \frac{3}{4}\left(\|\omega_{k}\|^2 +\|\theta_{k}\|^2+1\right).
% \end{align*}
\end{lem}
\begin{proof}
As a result of \eqref{eq:G_affinelybounded_D}, for any $k\geq 0$
\begin{align}
    \|\omega_{k+1}\|\hspace{-2pt}-\hspace{-2pt}\|\omega_{k}\|&\leq \|\omega_{k+1}\hspace{-2pt}-\hspace{-2pt}\omega_{k}\|\hspace{-2pt}=\hspace{-2pt}\|\beta_k G(\theta_{k+1},\omega_k,X_k)\|\hspace{-2pt}\leq\hspace{-2pt} D\beta_k\left(\|\theta_{k+1}\|\hspace{-2pt}+\hspace{-2pt}\|\omega_k\|\hspace{-2pt}+\hspace{-2pt}1\right).
    \label{lem:omega_k-omega_k-tau:ineq0}
\end{align}
% which leads to
% \begin{align*}
%     \|\omega_{k+1}\|&\leq(1+D\beta_k)\|\omega^{k}\|+D\beta_k (\|\theta_{k+1}\|+1).
% \end{align*}
Define $h_k=\|\omega_{k}\|+\|\theta_{k+1}\|$. We have for all $k\geq 1$
\begin{align*}
    h_k&=\|\omega_{k-1}+\beta_{k-1}G(\theta_k,\omega_{k-1},X_{k-1})\|+\|\theta_k+\alpha_k H(\theta_k,\omega_k,X_k)\|\notag\\
    &\leq \|\omega_{k-1}\|+D\beta_{k-1}(\|\theta_{k}\|+\|\omega_{k-1}\|+1)+\|\theta_k\|+B\alpha_k\notag\\
    &\leq (1+D\beta_{k-1})h_{k-1}+(B+D)\beta_{k-1}
\end{align*}
where the second inequality follows from \eqref{eq:G_affinelybounded_D} and Assumption \ref{assump:HG_smooth}, and the last inequality is due to $\alpha_k\leq\beta_k$ and the fact that $\{\beta_k\}$ is a decaying sequence.

Since $1+x \leq e^{x}$ for all $x\geq 0$, we have for all $k\geq\tau_k$ and $k-\tau_k\leq t\leq k$
\begin{align*}
    h_t&\leq (1+D\beta_{t-1})h_{t-1}+(B+D)\beta_{t-1}\notag\\
    &\leq (1+D\beta_{k-\tau_k})^{\tau_k+t-k} h_{k-\tau_k}+(B+D)\beta_{k-\tau_k}\sum_{t'=k-\tau_k}^{t-1}(1+D\beta_{k-\tau_k})^{t-t'-1}\notag\\
    &\leq (1+D\beta_{k-\tau_k})^{\tau_k} h_{k-\tau_k}+(B+D)\beta_{k-\tau_k}\tau_k(1+D\beta_{k-\tau_k})^{\tau_k}\notag\\
    &\leq e^{D\beta_{k-\tau_k}\tau_k}h_{k-\tau_k}+(B+D)\beta_{k-\tau_k}\tau_k e^{D\beta_{k-\tau_k}\tau_k}\leq 2h_{k-\tau_k}+\frac{1}{3},
\end{align*}
where the last inequality follows from the step size $2(B+D)\beta_{k-\tau_k}\tau_k\leq\frac{1}{3}\leq\log(2)$.
% 
Combining this inequality with \eqref{lem:omega_k-omega_k-tau:ineq0}, we have for all $k\geq\tau_k$
\begin{align*}
    &\|\omega_k-\omega_{k-\tau_k}\|\leq \sum_{t=k-\tau_k}^{k-1}\hspace{-3pt}\|\omega_{t+1}-\omega_t\| \leq D\hspace{-3pt}\sum_{t=k-\tau_k}^{k-1}\hspace{-3pt}\beta_{t}\left(h_t + 1\right) \leq D\beta_{k-\tau_k}\hspace{-3pt}\sum_{t=k-\tau_k}^{k-1}\hspace{-3pt}\big(2h_{k-\tau_k} + \frac{4}{3}\big) \notag\\
    &\leq\hspace{-2pt} 2D\beta_{k-\tau_k}\hspace{-2pt}\tau_k(\|\omega_{k-\tau_k}\| \hspace{-2pt}+\hspace{-2pt}\|\theta_{k-\tau_k+1}\|\hspace{-2.5pt}+\hspace{-2.5pt} \frac{2}{3}) \hspace{-2pt}\leq\hspace{-2pt} 2D\beta_{k-\tau_k}\hspace{-2pt}\tau_k(\|\omega_{k-\tau_k}\| \hspace{-2pt}+\hspace{-2pt}\|\theta_{k}\|\hspace{-2pt}+\hspace{-2pt}B\beta_{k-\tau_k}\hspace{-2pt}(\tau_k\hspace{-2pt}-\hspace{-2pt}1)\hspace{-2.5pt}+\hspace{-2.5pt} \frac{2}{3})\notag\\
    &\leq 2D\beta_{k-\tau_k}\tau_k\left(\|\omega_k-\omega_{k-\tau_k}\|+\|\omega_{k}\| +\|\theta_{k}\|+1\right).
\end{align*}
% where in the last inequality we use $2B\beta_{k-\tau_k}\tau_k\leq \frac{1}{3}$ again.
Re-arranging terms and again using the step size condition $2D\beta_{k-\tau_k}\tau_k\leq\frac{1}{3}$, we get
\begin{align*}
\|\omega_k-\omega_{k-\tau_k}\|&\leq 3D\beta_{k-\tau_k}\tau_k\left(\|\omega_{k}\| +\|\theta_{k}\|+1\right).
\end{align*}
\end{proof}

We now present Proposition~\ref{prop:auxiliary}, which reveals the effect of the decision variables on the convergence of the auxiliary variable.
\begin{prop}\label{prop:auxiliary}
Under Assumptions \ref{assump:HG_smooth}-\ref{assump:tv_bound}, we have for all $k\geq\Kcal$
\begin{align*}
    \mathbb{E}[\|z_{k+1}\|^2] &\leq (1\hspace{-2pt}-\hspace{-2pt}\frac{\lambda\beta_k}{2})\mathbb{E}[\|z_{k}\|^2]\hspace{-2pt}+\hspace{-2pt}C_2\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2\right]\hspace{-2pt}+\hspace{-2pt}\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}+C_2\tau_k^2\beta_{k-\tau_k}\beta_k.
\end{align*}
\end{prop}
\begin{proof}

We introduce a technical lemma that bounds the error in the auxiliary variable caused by the Markovian samples. We skip the proof of this lemma due to its similarity to that of Lemma~\ref{lem:Gamma_bound} and refer interested readers to the companion paper \cite{zeng2021two} for the full proof details.
\begin{lem}\label{lem:Lambda_bound}
    Recall the definition of $C_1$ in \eqref{notation:constant_C}. For any $k\geq\tau_k$, we have
    \begin{align*}
    \mathbb{E}[\langle z_k, \Delta G_k\rangle]\leq C_1\tau_k^2\beta_{k-\tau_k}\mathbb{E}\left[\|z_{k-\tau_k}\|^2+\|\theta_k\|^2+\|\omega_k\|^2+1\right].
\end{align*}
\end{lem}

Recall that $z_{k} = \omega_{k} - \omega^{\star}(\theta_{k})$. Using \eqref{alg:update_omega}, we have
\begin{align*}
    \|z_{k+1}\|^2
    % &=\|\omega_{k+1}-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    &= \|\omega_k+\beta_k G(\theta_{k+1},\omega_k, X_k)-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    &= \|\left(\omega_k-\omega^{\star}(\theta_k)\right)+\beta_k G(\theta_{k+1},\omega_k,X_k)+\left(\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\right)\|^2\notag\\
    % &= \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)\rangle+2\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle\notag\\
    % &\qquad + \|\beta_kG(\theta_{k+1},\omega_k,X_k)+ \omega^{\star}(\theta^k)-\omega^{\star}(\theta^{k+1})\|^2\notag\\
    &\leq \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)\rangle+2\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle\notag\\
    &\qquad + 2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2+2\|\omega^{\star}(\theta^k)-\omega^{\star}(\theta^{k+1})\|^2.
\end{align*}

% Recall from \eqref{eq:Delta_z_def} that $\Delta G_k = G(\theta_k,\omega_k,X_k)-\mathbb{E}_{\hat{X}\sim\mu_{\theta_k}}[G(\theta_k,\omega_k,\hat{X})]$. Using this in the equation above,
From the definition of $\Delta G_k$ in \eqref{eq:Delta_z_def},
\begin{align}
    \|z_{k+1}\|^2&\leq \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle+2\beta_k\langle z_k,G(\theta_{k},\omega_k,X_k)\rangle\notag\\
    &\quad+2\langle z_k,\omega^{\star}(\theta_k)\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k+1})\rangle\hspace{-2pt} + \hspace{-2pt}2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2\hspace{-2pt}+\hspace{-2pt}2\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    % &= \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle \rangle\notag\\
    % &\quad+ 2\beta_k\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle+2\beta_k\langle z_k,\Delta G_{k}\rangle \hspace{-2pt}+\hspace{-2pt} 2\langle z_k,\omega^{\star}(\theta_k)\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k+1})\rangle  \notag\\ 
    % &\quad + 2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2 + 2\|\omega^{\star}(\theta^k)-\omega^{\star}(\theta^{k+1})\|^2\notag\\
    &\leq \|z_k\|^2+2\beta_k\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle\rangle\notag\\
    &\quad + 2\beta_k\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle \hspace{-2pt}+\hspace{-2pt} 2\beta_k\langle z_k,\Delta G_{k}\rangle + 2\langle z_k,\omega^{\star}(\theta_k)\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k+1})\rangle \notag\\
    &\quad+2\beta_k^2\left\|G(\theta_{k+1},\omega_k,X_k)\right\|^2+2L^2 B^2\alpha_k^2,
    \label{prop:auxiliary_eq1}
\end{align}
where the second inequality applies Assumption \ref{assump:HG_smooth} and \eqref{alg:update_theta}, i.e.,
\begin{equation}
 \|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\|^2 \leq  L^2 \|\theta_k-\theta_{k+1}\|^2= L^2\|\alpha_k H(\theta_k,\omega_k,X_k)\|^2 \leq L^2B^2\alpha_k^2.
    \label{prop:auxiliary_eq1.5}
\end{equation}
We next analyze each term on the right-hand side of \eqref{prop:auxiliary_eq1}. First, using the relation $\langle 2v_1,v_2\rangle\leq c\|v_1\|^2+\frac{1}{c}\|v_2\|^2$ for any vectors $v_1,v_2$ and scalar $c>0$, we bound the second term of \eqref{prop:auxiliary_eq1}
\begin{align}
    &\langle z_k,\hspace{-1pt}G(\theta_{k+1},\omega_k,\hspace{-1pt}X_k)\hspace{-2pt}-\hspace{-2pt}G(\theta_{k},\omega_k,\hspace{-1pt}X_k)\rangle\hspace{-2pt}\leq\hspace{-2pt} \frac{\lambda}{4}\|z_k\|^2\hspace{-2pt}+\hspace{-2pt}\frac{1}{\lambda}\|G(\theta_{k+1},\omega_k,\hspace{-1.5pt}X_k)\hspace{-2pt}-\hspace{-2pt}G(\theta_{k},\omega_k,\hspace{-1.5pt}X_k)\|^2\notag\\
    &\leq \frac{\lambda}{4}\|z_k\|^2+\frac{L^2}{\lambda}\|\theta_{k+1}-\theta_{k}\|^2 \leq \frac{\lambda}{4}\|z_k\|^2+\frac{L^2 B^2\alpha_k^2}{\lambda},\label{prop:auxiliary_eq1a}
\end{align}
where the second inequality follows from the Lipschitz continuity of $G$ and the last inequality is due to \eqref{prop:auxiliary_eq1.5}. Similarly, we consider the fifth term of \eqref{prop:auxiliary_eq1}
\begin{align}
    &2\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle\leq \frac{\beta_k\lambda}{2}\|z_k\|^2+\frac{2}{\lambda\beta_k}\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\|^2\notag\\
    &\leq \frac{\beta_k\lambda}{2}\|z_k\|^2+\frac{2L^2}{\lambda\beta_k}\|\theta_k-\theta_{k+1}\|^2\leq \frac{\beta_k\lambda}{2}\|z_k\|^2+\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}.\label{prop:auxiliary_eq1b}
\end{align}
Next, using Assumption \ref{assump:stronglymonotone_G} and $z_{k} = \omega_{k} - \omega^{\star}(\theta_{k})$ we consider the third term of \eqref{prop:auxiliary_eq1}
\begin{align}
    2\beta_k\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle \leq -2\lambda\beta_k\|z_k\|^2.\label{prop:auxiliary_eq1c}
\end{align}
By \eqref{eq:G_affinelybounded_D}  and \eqref{alg:update_theta} we have
\begin{align}
\|G(\theta_{k+1},\omega_{k},X_{k})\|^2 \hspace{-2pt}\leq \hspace{-2pt}2D^2 \big(\|\theta_{k+1}\| \hspace{-2pt}+\hspace{-2pt} \|\omega_{k}\| + 1\big)^2\hspace{-2pt}\leq \hspace{-2pt}  2D^2 \big(\|\theta_{k}\| \hspace{-2pt}+\hspace{-2pt} B\alpha_{k} + \|\omega_{k}\| \hspace{-2pt}+\hspace{-2pt} 1\big)^2.\label{prop:auxiliary_eq1d}
% &\quad\leq 2D^2\beta_{k}^2 \big(\|\theta_{k}\| + B\alpha_{k} + \|\omega_{k}-\omega^{\star}(\theta_{k})\| + \|\omega^{\star}(\theta_{k})\| + 1\big)^2\notag\\
% &\quad \leq 2D^2\beta_{k}^2 \big((1+D)\|\theta_{k}\| + B\alpha_{k} + \|z_{k}\| + D + 1\big)^2,
\end{align}
Taking the expectation on both sides of \eqref{prop:auxiliary_eq1} and using \eqref{prop:auxiliary_eq1a}--\eqref{prop:auxiliary_eq1d} and Lemma \ref{lem:Lambda_bound}
\begin{align}
    \mathbb{E}[\|z_{k+1}\|^2]
    % &\leq \mathbb{E}[\|z_k\|^2]+2\beta_k\mathbb{E}[\langle z_k,G(\theta_{k+1},\omega_k,X_k)-G(\theta_{k},\omega_k,X_k)\rangle]\notag\\
    % &\quad+2\beta_k\mathbb{E}[\langle z_k,\mathbb{E}_{\hat{X}\sim\mu_{\theta_{k}}}[G(\theta_{k},\omega_k,\hat{X})]\rangle]+2\beta_k\mathbb{E}[\left\langle z_k, \Delta G_k\right\rangle]\notag\\
    % &\quad+2\mathbb{E}[\langle z_k,\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k+1})\rangle]+6D^2\beta_k^2(\|\theta_{k+1}\|^2+\|\omega_k\|^2+1)+2L^2 B^2 \alpha_k^2\notag\\
    &\leq \mathbb{E}[\|z_k\|^2]+\frac{\beta_k\lambda}{2}\mathbb{E}[\|z_k\|^2]+\frac{2L^2 B^2 \beta_k\alpha_k^2}{\lambda}+\frac{\beta_k\lambda}{2}\mathbb{E}[\|z_k\|^2]+\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}\notag\\
    &\quad-2\lambda\beta_k\mathbb{E}[\|z_k\|^2]+C_1\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k-\tau_k}\|^2+\|\theta_k\|^2+\|\omega_k\|^2+1\right]\notag\\
    &\quad + 2D^2\beta_{k}^2 \big(\|\theta_{k}\| + B\alpha_{k} + \|\omega_{k}\| + 1\big)^2 + 2L^2 B^2\alpha_k^2\notag\\
    &\leq (1-\lambda\beta_k)\mathbb{E}[\|z_k\|^2]+C_1\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k-\tau_k}\|^2\right]\notag\\
    &\quad+(C_1+8D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2+\|\omega_k\|^2\right]\notag\\
    &\quad+\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}+(C_1+32D^2+\frac{2L^2 B^2}{\lambda}+2L^2 B^2)\tau_k^2\beta_{k-\tau_k}\beta_k,
    \label{prop:auxiliary_eq2}
\end{align}
where the last inequality uses $\alpha_k\leq\beta_k$ and $B\alpha_k\leq 1$.  Note that $\|z_{k-\tau_k}\|^2$ obeys
\begin{align*}
    \|z_{k-\tau_k}\|^2&=\|z_k-(\omega_k-\omega_{k-\tau_k})+(\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k-\tau_k}))\|^2\notag\\
    &\leq 3\left(\|z_k\|^2+\|\omega_k-\omega_{k-\tau_k}\|^2+\|\omega^{\star}(\theta_k)-\omega^{\star}(\theta_{k-\tau_k})\|^2\right)\notag\\
    &\leq 3\|z_k\|^2+\frac{9}{4}\left(\left\|\omega_{k}\right\|^{2}+\left\|\theta_{k}\right\|^{2}+1\right)+L^2\|\theta_{k}-\theta_{k-\tau_k}\|^2\notag\\
    &\leq 3\left(\|z_k\|^2+\|\omega_{k}\|^{2}+\|\theta_{k}\|^{2}\right)+L^2 B^2\tau_k^2\alpha_{k-\tau_k}^2+\frac{9}{4}\notag\\
    &\leq 3\left(\|z_k\|^2+\|\omega_{k}\|^{2}+\|\theta_{k}\|^{2}+1\right),
\end{align*}
where the second inequality is due to Lemma \ref{lem:omega_k-omega_k-tau} and the Lipschitz continuity of $\omega^{\star}$, and the last inequality follows from the step size condition $L B\tau_k\alpha_{k-\tau_k}\leq\frac{1}{6}$. Substituting the preceding relation into \eqref{prop:auxiliary_eq2}, we have for all $k\geq\tau_k$
\begin{align}
    \mathbb{E}[\|z_{k+1}\|^2] &\leq (1-\lambda\beta_k)\mathbb{E}[\|z_k\|^2]+3C_1\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k}\|^2\right]\notag\\
    &\quad+(4C_1+8D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2+\|\omega_k\|^2\right]\notag\\
    &\quad+\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}+(4C_1+32D^2+\frac{2L^2 B^2}{\lambda}+2L^2 B^2)\tau_k^2\beta_{k-\tau_k}\beta_k\notag\\
    &\leq (1-\lambda\beta_k)\mathbb{E}[\|z_k\|^2]+(11C_1+16D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|z_{k}\|^2\right]\notag\\
    &\quad+(4D^2+1)(4C_1+8D^2)\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2\right]+\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}\notag\\
    &\quad+((4D^2+1)(4C_1+32D^2)+\frac{2L^2 B^2}{\lambda}+2L^2 B^2)\tau_k^2\beta_{k-\tau_k}\beta_k,
    \label{prop:auxiliary_eq2.5}
\end{align}
where in the last inequality we use \eqref{eq:G_affinelybounded_D} to derive 
\begin{align*}
    \|\omega_k\|^2\hspace{-2pt}\leq \hspace{-2pt}2\|\omega_{k}\hspace{-2pt}-\hspace{-2pt}\omega^{\star}(\theta_{k})\|^2\hspace{-2pt}+\hspace{-2pt}2\|\omega^{\star}(\theta_{k})\|^2\hspace{-2pt}\leq\hspace{-2pt} 2\|z_k\|^2\hspace{-2pt}+\hspace{-2pt}2D^2(\|\theta_k\|\hspace{-2pt}+\hspace{-2pt}1)^2\hspace{-2pt}\leq\hspace{-2pt} 2\|z_k\|^2\hspace{-2pt}+\hspace{-2pt}4D^2(\|\theta_k\|^2\hspace{-2pt}+\hspace{-2pt}1).
\end{align*}
By the choice of the step size we have $(11C_1+16D^2)\tau_k^2\beta_{k-\tau_k}\leq\frac{\lambda}{2}$. Thus, using the constant $C_2$ defined in \eqref{notation:constant_C}, \eqref{prop:auxiliary_eq2.5} implies
\begin{align*}
    \mathbb{E}[\|z_{k+1}\|^2] \leq(1-\frac{\lambda\beta_k}{2})\mathbb{E}[\|z_k\|^2]+C_2\tau_k^2\beta_{k-\tau_k}\beta_k\mathbb{E}\left[\|\theta_k\|^2+1\right]+\frac{2L^2 B^2 \alpha_k^2}{\lambda\beta_k}.
\end{align*}
\end{proof}

As mentioned earlier, the update of the auxiliary variable occurs at a faster time scale, i.e.\ $\alpha_{k} \ll \beta_{k}$, in order to provide a more accurate gradient for the update of $\theta_k$.
Propositions~\ref{prop:pl_nonconvex} and \ref{prop:auxiliary} show that the convergence of the decision variable and the auxiliary variable forms a coupled dynamical system that evolves under two different rates. To characterize the  coupling of the two iterates and analyze the finite-time complexity, we consider the following Lyapunov function 
\begin{equation*}
    V(\theta_{k},\omega_{k}) = \Eset[f(\theta_{k})-f^{\star}] + (\alpha_{k}/\beta_{k})\Eset[\|\omega_{k}-\omega^{\star}(\theta_{k})\|^2].    
\end{equation*}
We will derive the finite-time convergence rate of $V(\theta_k,\omega_k)$ to 0, which immediately translates to the convergence rates for $\Eset[f(\theta_{k})-f^{\star}]$ and $\Eset[\|\omega_{k}-\omega^{\star}(\theta_{k})\|^2]$.





\subsection{Two-Time-Scale Lemma}
\label{sec:lyapunov_lemma}
Although we analyze the performance of our algorithm for different types of objective functions and with different convergence metrics, these analyses eventually reduce to the study of two coupled inequalities. The dynamics of these two inequalities happen on different time scales determined by the two step sizes used in our algorithm. 
%
In this section we present a general result, which we call the two-time-scale lemma, that characterizes the behavior of these coupled inequalities. \looseness=-1
% This lemma gives us a tool for a unified analysis for different types of objectives $f$, and may be of further interest to the study of the finite-time performance of multiple-time-scale dynamical systems apart from those considered in this paper. 






\begin{lem}\label{lem:lyapunov}
    Let $\{a_k,\, b_k,\,c_k,\,d_k,\,e_k,\,f_k\}$ be non-negative 
    % and constant 
    sequences satisfying $\frac{a_{k+1}}{d_{k+1}}\leq\frac{a_{k}}{d_{k}} < 1$, for all $k\geq0$.
    Let $\{x_k\}, \{y_k\}$ be two non-negative sequences. We consider two settings on their dynamics. 
\begin{enumerate}[leftmargin = 4.5mm]
    \item  Suppose that $x_{k},y_{k}$ satisfy the following coupled inequalities
    \begin{align}
    x_{k+1}\leq(1-a_k)x_k+b_k y_k+c_k,\quad y_{k+1}\leq(1-d_k)y_k+e_k x_k+f_k.\label{lem:lyapunov:sc:def}
    \end{align}
    In addition, assume that there exists a constant $A\in\mathbb{R}$ such that  
    \begin{align}
    Aa_k-b_k-\frac{A a_k^2}{d_k}\geq 0\quad \text{and}\quad  \frac{A e_k}{d_{k}}\leq\frac{1}{2}, \quad \text{for all } k\geq0. \label{lem:lyapunov:sc:def3}
    \end{align}
    Then we have  for all $0 \leq \tau \leq k$
    \begin{align*}
    x_k&\leq (x_{\tau}+\frac{A a_{\tau} }{d_{\tau}}y_{\tau})\prod_{t=\tau}^{k-1}(1-\frac{a_t}{2})+\sum_{\ell=\tau}^{k-1}\Big(c_{\ell}+\frac{A a_{\ell} f_{\ell}}{d_{\ell}}\Big) \prod_{t=\ell+1}^{k-1}(1-\frac{a_t}{2}).
    \end{align*}
    
    \item  Suppose that $\{x_k,y_k\}$ satisfy the following coupled inequalities
    \begin{align}
    x_{k+1}\leq(1+a_k)x_k+b_k y_k+c_k,\quad y_{k+1}\leq(1-d_k)y_k+e_k x_k+f_k.\label{lem:lyapunov:def}
    \end{align}    
    $\{u_k\}$ is a non-negative sequence such that
    \begin{align}
        u_k\leq(1+a_k)x_k-x_{k+1}+b_k y_k+c_k,\label{lem:lyapunov:def3}
    \end{align}
    then we have for any $0 \leq \tau \leq k$
    \begin{align*}
    \sum_{t=\tau}^{k}u_t \leq \Big(1+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})e^{\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})}\Big)\Big(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\Big).
\end{align*}
\end{enumerate}    
\end{lem}
\begin{proof}
Case 1) Consider $V_k=x_k+\frac{A a_k}{d_k}y_k$. From the second equation in \eqref{lem:lyapunov:sc:def},
\begin{align*}
    \frac{A a_{k+1}}{d_{k+1}}y_{k+1} &\leq \frac{A a_{k}}{d_{k}}y_{k+1} \leq \frac{A a_{k}}{d_{k}}\left((1-d_k)y_k+e_k x_k+f_k\right)\notag\\
    &= (1-a_k)\frac{A a_{k}}{d_{k}}y_k+(a_k-d_k)\frac{A a_{k}}{d_{k}}y_k+\frac{A a_{k}e_k x_k}{d_{k}}+\frac{A a_{k} f_k}{d_{k}}.
\end{align*}
Combining this with the first inequality of \eqref{lem:lyapunov:sc:def} yields
\begin{align*}
    V_{k+1}&=x_{k+1}+\frac{A a_{k+1}}{d_{k+1}}y_{k+1}\notag\\
    &\leq (1\hspace{-2pt}-\hspace{-2pt}a_k)x_k\hspace{-2pt}+\hspace{-2pt}b_k y_k\hspace{-2pt}+\hspace{-2pt}c_k\hspace{-2pt}+\hspace{-2pt}(1\hspace{-2pt}-\hspace{-2pt}a_k)\frac{A a_{k}}{d_{k}}y_k\hspace{-2pt}+\hspace{-2pt}(a_k\hspace{-2pt}-\hspace{-2pt}d_k)\frac{A a_{k}}{d_{k}}y_k\hspace{-2pt}+\hspace{-2pt}\frac{A a_{k}e_k x_k}{d_{k}}\hspace{-2pt}+\hspace{-2pt}\frac{A a_{k} f_k}{d_{k}}\notag\\
    &= (1-a_k)\left(x_k+\frac{A a_k y_k}{d_k}\right)+\left(\frac{A a_k^2}{d_k}-A a_k+b_k\right)y_k+c_k+\frac{A a_{k}e_k x_k}{d_{k}}+\frac{A a_{k} f_k}{d_{k}}\notag\\
    &\leq (1-a_k)V_k+\frac{a_k}{2}x_k+c_k+\frac{A a_{k} f_k}{d_{k}}\leq (1-\frac{a_k}{2})V_k+c_k+\frac{A a_{k} f_k}{d_{k}},
\end{align*}
where the second inequality follows from \eqref{lem:lyapunov:sc:def3}.
Applying this relation recursively,
\begin{align*}
    x_k&\leq V_k\leq V_{\tau}\prod_{t=\tau}^{k-1}(1-\frac{a_t}{2})+\sum_{\ell=\tau}^{k-1}\left(c_{\ell}+\frac{A a_{\ell} f_{\ell}}{d_{\ell}}\right) \prod_{t=\ell+1}^{k-1}(1-\frac{a_t}{2})\\
    &\leq (x_{\tau}+\frac{A a_{\tau} }{d_{\tau}}y_{\tau})\prod_{t=\tau}^{k-1}(1-\frac{a_t}{2})+\sum_{\ell=\tau}^{k-1}\left(c_{\ell}+\frac{A a_{\ell} f_{\ell}}{d_{\ell}}\right) \prod_{t=\ell+1}^{k-1}(1-\frac{a_t}{2}).
\end{align*}


Case 2) Re-arranging the second inequality of \eqref{lem:lyapunov:def} and multiplying by $\frac{b_k}{d_k}$, we get\looseness=-1
\begin{align*}
    b_k y_k\leq \frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+\frac{b_k e_k x_k}{d_k}+\frac{b_k f_k}{d_k}.
\end{align*}
Plugging this inequality into the first inequality of \eqref{lem:lyapunov:def} yields
\begin{align}
    x_{k+1}&\leq(1+a_k)x_k+c_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+\frac{b_k e_k x_k}{d_k}+\frac{b_k f_k}{d_k}\notag\\
    &\leq(1+g_k)x_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+c_k+\frac{b_k f_k}{d_k},
    \label{lem:lyapunov:eq3}
\end{align}
where we define $g_k=a_k+\frac{b_k e_k}{d_k}$.
Since $1+c\leq\exp(c)$ for any scalar $c>0$, we have
\begin{align}
    x_{k+1}
    % &\leq(1+a_k+\frac{b_k e_k}{d_k})x_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+c_k+\frac{b_k f_k}{d_k}\notag\\
    &\leq\exp(g_k)x_k+\frac{b_k}{d_k}y_k-\frac{b_k}{d_k}y_{k+1}+c_k+\frac{b_k f_k}{d_k}\notag\\
    &\leq\exp(\sum_{t=\tau}^{k}g_t)x_{\tau}+\exp\big(\sum_{t=\tau}^{k}g_t\big)\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
    &\leq \exp(\sum_{t=\tau}^{k}g_t)\Big(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\Big),
    \label{lem:lyapunov:eq4}
\end{align}
where the second inequality applies the first inequality recursively. 
% This bound implies
% \begin{align}
%     \max_{\tau\leq t\leq k}x_t &\leq \exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))x_{\tau}\notag\\
%     &\hspace{20pt}+\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
%     &\leq \exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right).
%     \label{lem:lyapunov:eq4}
% \end{align}
The inequalities \eqref{lem:lyapunov:eq3}, \eqref{lem:lyapunov:eq4}, and \eqref{lem:lyapunov:def3} together imply
\begin{align*}
    \sum_{t=\tau}^{k}u_t&\leq \sum_{t=\tau}^{k}(x_t-x_{t+1})+\big(\hspace{-2pt}\max_{\tau\leq t\leq k}x_t\big)\hspace{-2pt}\sum_{t=\tau}^{k}g_t+\hspace{-2pt}\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
    &\leq x_{\tau}\hspace{-1pt}+\hspace{-2pt}\sum_{t=\tau}^{k}g_t\exp\big(\sum_{t=\tau}^{k}g_t\big)\Big(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\Big)+\frac{b_{\tau}}{d_{\tau}}y_{\tau}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\notag\\
    &=\left(1+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\right)\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right).
\end{align*}
% \begin{align*}
%     \sum_{t=\tau}^{k}u_t &\leq \sum_{t=\tau}^{k}(x_t-x_{t+1})+\big(\hspace{-2pt}\max_{\tau\leq t\leq k}x_t\big)\hspace{-2pt}\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))+\hspace{-2pt}\sum_{t=\tau}^{k}\left(\frac{b_t}{d_t}(y_t-y_{t+1})+c_t+\frac{b_t f_t}{d_t}\right)\notag\\
%     &\leq x_{\tau}+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right)\notag\\
%     &\hspace{20pt}+\frac{b_{\tau}}{d_{\tau}}y_{\tau}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\notag\\
%     &=\left(1+\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t})\exp(\sum_{t=\tau}^{k}(a_t+\frac{b_t e_t}{d_t}))\right)\left(x_{\tau}+\frac{b_{\tau}y_{\tau}}{d_{\tau}}+\sum_{t=\tau}^{k}(c_t+\frac{b_t f_t}{d_t})\right).
% \end{align*}
\end{proof}

Lemma \ref{lem:lyapunov} studies the behavior of the two interacting sequences $\{x_k\}$ and $\{y_k\}$ that have generic structure. In our analysis, properly selected convergence metrics on $\theta_k$ and $\omega_k$ evolve as $x_k$ and $y_k$ above, respectively, according to \eqref{lem:lyapunov:sc:def} for strongly convex and P\L~functions and \eqref{lem:lyapunov:def} for non-convex functions, while the sequences $\{a_k,\, b_k,\,c_k,\,d_k,\,e_k,\,f_k\}$ are ratios and products of the step sizes $\{\alpha_k\}$ and $\{\beta_k\}$.\looseness=-1





